Abstract Transducers

Several abstract machines that operate on symbolic input alphabets have been proposed in the last decade, for example, symbolic automata or lattice automata. Applications of these types of automata include software security analysis and natural language processing. While these models provide means to describe words over infinite input alphabets, there is no considerable work on symbolic output (as present in transducers) alphabets, or even abstraction (widening) thereof. Furthermore, established approaches for transforming, for example, minimizing or reducing, finite-state machines that produce output on states or transitions are not applicable. A notion of equivalence of this type of machines is needed to make statements about whether or not transformations maintain the semantics. We present abstract transducers as a new form of finite-state transducers. Both their input alphabet and the output alphabet is composed of abstract words, where one abstract word represents a set of concrete words. The mapping between these representations is described by abstract word domains. By using words instead of single letters, abstract transducers provide the possibility of lookaheads to decide on state transitions to conduct. Since both the input symbol and the output symbol on each transition is an abstract entity, abstraction techniques can be applied naturally. We apply abstract transducers as the foundation for sharing task artifacts for reuse in context of program analysis and verification, and describe task artifacts as abstract words. A task artifact is any entity that contributes to an analysis task and its solution, for example, candidate invariants or source code to weave.

==> text/background.tex <==
\chapter{Background}
\label{cha:background}%

This work introduces existing concepts and techniques for 
program analysis and software model checking that are the 
foundation of this work.
Please note that definitions of different terms vary within 
the community.
We use the formalisms and definitions that fit best for this work:
Readers that are already familiar with the field of program
analysis and model checking should take notice of the definitions, 
formalisms, and notions we use.

Possible sources for further information on basic concepts are the 
\emph{Handbook of Practical Logic and Automated Reasoning}~\cite{LogicHandbook},
the \emph{Handbook of Model Checking}~\cite{Handbook},
and the \emph{Principles of Program Analysis}~\cite{ProgramAnalysisNielson}.

\section{Program Representation}

Before we introduce concepts for program analysis, we introduce 
formalisms and concepts to represent the \emph{syntactical} 
structure of programs and do not focus on their semantics yet.

\subsection{Language and Word}
\newcommand{\abstconcat}{\ensuremath{\varotimes}\xspace}%
\newcommand{\prefixof}{\ensuremath{\preceq}\xspace}%
\newcommand{\alphabet}{\ensuremath{\Sigma}\xspace}%
\newcommand{\words}{\ensuremath{\alphabet^*}\xspace}%
\newcommand{\infinitewords}{\ensuremath{\alphabet^{\omega}}\xspace}%
\newcommand{\eitherwords}{\ensuremath{\alphabet^{\square}}\xspace}%
\newcommand{\allwords}{\ensuremath{\alphabet^{\infty}}\xspace}%
\newcommand{\finitewords}{\ensuremath{\words}\xspace}%
\newcommand{\word}{\ensuremath{\bar{\sigma}}\xspace}%
\newcommand{\worda}{\ensuremath{\bar{a}}\xspace}%
\newcommand{\wordb}{\ensuremath{\bar{b}}\xspace}%
\newcommand{\wordc}{\ensuremath{\bar{c}}\xspace}%
\newcommand{\letter}{\ensuremath{\sigma}\xspace}%
\label{concept:concat}%
\label{concept:language}%
\label{concept:transduction}%
We take a language-theoretic approach for formalizing many of the 
concepts and techniques that we present in this work.
\recap{Word}
The set of all \emph{finite words} over an \emph{alphabet}~$\Sigma$ 
is denoted by~$\alphabet^*$, which is a 
free monoid~$\alphabet^* = (\alphabet, \concat, \epsilon)$, 
also known as Kleene star, where 
\emph{concatenation}~$\concat: \words \times \words \rightarrow \words$
is its binary operator and its neutral element~$\epsilon$ is 
the \emph{empty word}.
A \emph{word}~$\bar{\sigma}$ is a sequence~$\langle \sigma_1, \ldots, \sigma_n \rangle$ 
of symbols from the alphabet.
The concatenation $W_1 \concat W_2$ of two collections $W_1 \subseteq \alphabet^*$ 
and~$W_2 \subseteq \alphabet^*$ of words is conducted pairwise, 
and is defined as $W_1 \concat W_2 := \{ \bar{w_1} \concat \bar{w_2} \: | \;  \bar{w_1} \in W_1 \land \bar{w_2} \in W_2 \}$.
The set of all symbols in a word~$\bar{s}$ is denoted 
by~$\alphabet(\bar{s}) \subseteq \alphabet$.
The \emph{length}~$|\bar{\sigma}|$ of a word~$\bar{\sigma}$
is its number of subsequent symbols; the empty word 
has length~$|\epsilon| = |\langle \rangle| = 0$.
Given two words~$\bar{\sigma} = \langle \sigma_1, \ldots, \sigma_n \rangle$ 
and $\bar{\tau} = \langle \tau_1, \ldots, \tau_m \rangle$,
the concatenation~$\bar{\sigma} \concat \bar{\tau}$ 
results in the word~$\bar{c} = \langle \sigma_1, \ldots, \sigma_n, 
\tau_1, \ldots, \tau_m \rangle$ 
with length~$|\bar{c}| = |\bar{\sigma}| + |\bar{\tau}|$.

\recap{Prefix}
A word~$\word_a$ is \emph{prefix} of another word~$\word_b$, that is,
it is element~$(\word_a, \word_b) \in \prefixof$ of the prefix
relation~$\prefixof$, if there exists a \emph{suffix}~$\word_s \in \Sigma^*$ 
such that~$\word_b = \word_a \concat \word_s$.
Given a word~$\bar{s} = \langle s_1, \ldots, s_n \rangle$, 
the~\emph{prefix operator}~$\prefix: \alphabet^* \rightarrow \alphabet^*$ returns 
a new word without the~\emph{last symbol}~$s_n = \last(\pathsegment)$.

\recap{Finite and Infinite}
Finitely long words over an alphabet~$\alphabet$ are denoted 
by~$\finitewords$, the \emph{infinitely long} ones are denoted 
by~$\infinitewords$.
The set of all words is denoted by~$\allwords = \finitewords \cup \infinitewords$~\cite{LodingTollkoetter2016}, 
with the \emph{infinite iteration}~$\cdot^\omega$ and 
the \emph{finite iteration}~$\cdot^*$.

\recap{Language}
The set of all words over an alphabet~$\Sigma$ that is 
described by a structure~$S$ and that are considered well-formed 
regarding certain production rules is called 
\emph{language}~$\langua(S) \subseteq \Sigma^\infty$ of $S$.
The \emph{empty word language} $\{ \epsilon \}$ consists of 
the empty word~$\epsilon$ only, the \emph{empty language} 
corresponds to the empty set~$\{ \}$.

\subsection{Program}
\label{concept:complocation}%
\label{concept:program}%
\label{concept:ops}%
We formalize programs based on several building blocks: 
the set of all typed~\emph{data locations}~$\datalocs$, 
the set of all \emph{control locations}~$\locs$,
the set of all \emph{program operations}~$\ops$,
and the set of all \emph{control transitions}~$G = 
\locations \times \ops \times \locations$.

A data location~$\dataloc \in \datalocs$ corresponds to a specific 
memory cell on the heap or stack.
\recap{Control Locations}
The set of control locations (\emph{program locations}) corresponds 
to possible values of the \emph{program counter} register, 
which is also known as the~\emph{instruction pointer}.
A control location~$\location \in \locations$ is a point in a 
program where the value of all memory locations can be 
observed~\cite{ClarkeEtal1992}.
Control locations help to identify common points in the control flow.
We use a \emph{special data location}~$\pc \in \datalocs$ that 
holds the current position in the control flow: It represents 
the program counter register.
\recap{Compound Locations}
A control location can be~\emph{compound}: 
A composite~$(\location_p, \location_c) \in \locations$ is composed 
of a \emph{major control location}~$\location_p \in \locations$ 
and a \emph{minor control location}~$\location_c \in \locations$.
Please note that we add attributes to control locations along 
with this work, which might give control locations further semantics.

\recap{Program Operations}
The set of program operations~$\ops = \opsassume \: \cup \: \opsnonassume$ 
consists of assignments~\opsassign and assumes~\opsassume on 
data locations; we model the neutral program 
operation~$\neutralop \in \opsassume$ as an 
assumption that always evaluates to \true.
\recap{Neutral Program Operation}
Furthermore, we assume that the operation~$\neutralop$ does not
influence any temporal properties of the program under analysis,
that is, a control-flow transition with the program operation~$\neutralop$
is dual to an $\epsilon$-move in a NFA~\cite{Sipser}.
Each operation~$\op \in \ops$ is represented by an abstract syntax tree.

A~\emph{program} is a finite sequence~\program of program statements, where 
one~\emph{program statement} is compound of a set of program operations and 
can---depending on its evaluation result---jump to different control locations.
\recap{Program Concerns}
A program is composed~(written) to contribute to particular program concerns.
The set~\concerns denotes all \emph{program concerns};
each control transition can contribute to a set of different concerns.

\subsection{Control Flow Automaton}
\label{concept:cfa}%
We represent a program~\program by 
a~\emph{control-flow automaton}~\cite{LazyAbstraction}%
~$\cfa_\program = (\locations_\program, \controlflows_\program, \location_0)$,
with a set~$\locations_\program \subseteq \locations$ of control 
locations, a \emph{control transition 
relation}~$\controlflows_\program \subseteq \controlflows$ 
of possible \emph{control flows} (transitions) between the 
control locations,
and the initial control location~$\location_0 \in \locations_\program$.
The set of~$\locations_\final$ of \emph{final control locations}~(states) 
is defined implicitly: It is the set of control locations where the CFA 
relinquishes its control~\cite{LustigVardi2013}.

\recap{Control Path}
A \emph{sequence of control transitions}~$\vstart g_1, \ldots \vend \in \controlflows^\infty$ 
is \emph{well-formed} regarding a control transition relation~$\controlflows_r \subseteq \controlflows$
if~$g_1 \in \controlflows_r$ and for all~${i \in \langle 2, \ldots \rangle}$, 
with~$g_{i-1} = (\cdot, \cdot, \location) \in \controlflows_r$ 
holds true that $g_i = (\location, \cdot, \cdot) \in \controlflows_r$.
A finite sequence of control transitions can also be written 
as~$\location_1 \transconc{op_1} \location_2 \ldots \transconc{\op_n} \location_{n+1}$.
A~\emph{control path}---also referred to as \emph{path segment}---is a 
well-formed sequence of control transitions;
a \emph{program control path} (or \emph{program trace}) is a control 
path that starts in the initial control location~$\location_0 \in \locations_\program$ 
of a program and its \cfa.
Please note that we sometimes use the notion of control path 
in a projected form, that is, either as a 
sequence~$\controlpath = \vstart l_0, \ldots \vend \in \locations^*$  
of control locations
or as a sequence~$\controlpath = \vstart op_1, \ldots \vend \in \ops^*$
of program operations.

The \emph{transitive closure} of a set of 
locations~$M \subseteq L$ regarding a 
transition relation~$\controlflows_r$ is denoted 
by~$M^+ \subseteq L \times L$, 
\recap{Closure}
that is, for all pairs~$(l_1, l_2) \in M^+$ exists a 
well-formed control path from~$l_1$ to~$l_2$ on~$\controlflows_r$.
A set of locations~$M \subseteq L$ is said to be~\emph{connected} 
if there exists a control path between every pair of 
locations in~$M$, that is, for all~$l_1, l_2 \in M$, 
either $(l_1,l_2) \in M^+$ or $(l_2, l_1) \in M^+$.

\newcommand{\functions}{\ensuremath{F}\xspace}%
\newcommand{\function}{\ensuremath{f}\xspace}%
\newcommand{\functionof}{\ensuremath{\functions}\xspace}%
The set~$\functions$ represents \emph{all functions} of a program.
\recap{Function Locations}
Given a function~$f \in F$, the set~$L(f) \subseteq L$ represents all control locations
that belong to the function~$f$, the set~$\controlflows(f) = \{ g \,|\, (l_1, \cdot, l_2) \in \controlflows \land l_2 \in L(f) \}$ 
represents all transitions that lead to a location in~$f$.
Given a control location~$l \in L$, the function $F(l) \in F$ represents the function
to that location~$l$ belongs to.

\subsection{Language of a Program}
\label{sec:languageofprograms}%
The \emph{language of a program}~\program and its control-flow automaton~$\cfa_\program$ 
is the set of all its program control 
paths~$\langua(\program) = \langua(\cfa_\program) \subseteq \controlflows^\infty$, that is,
the set of sequences of control transitions that are well-formed regarding the 
control transition relation~$\controlflows_\program$.
The language~$\langua_\ops(\program) \subseteq \ops^\infty$ is a projection 
of~$\langua(\program)$ with words over program operations only.
The language~$\langua_\locations(\program) \subseteq \locations^\infty$ is 
a projection of~$\langua(\program)$ with words over control locations only.

\begin{figure}[t]
{\smaller
\begin{align*}
    program &= \; \{ \; statement \; ";" \; \} \; ; \\
    statement &= declare \; | \; assign \; | \; condjump  ; \\
    condjump &= \srccode{"if"} \; assume \; \srccode{"goto"} \; stmtno \; \srccode{"else"} \; stmtno \; ; \\
    declare &= \; ? \; \texttt{declaration of arrays with different types and lengths} \; ? \; ; \\
    assign &= \; ? \; \texttt{assignment to a array cell from a given expression} \; ? \; ; \\
    assume &= \; ? \; \texttt{an expression that evaluates to the type 'bool'} \; ? \; ; \\
    stmtno &= \; ? \; \texttt{an unique identifier $\in \mathbb{N}_0$ of a} \; statement \; ? \; ; 
\end{align*}
}
\caption{The Turing-complete Pseudo Programming Language (PPL) \\and its pseudo grammar}
\label{fig:turing}
\end{figure}

Figure~\ref{fig:turing} shows a basic Turing-complete language without functions, 
to illustrate the basic complexities we have to cope with.
You can assume that functions are inlined and recursions are 
transformed to loops.
The number of words of a (imperative) program is determined 
by its control structure
and the transition system that is implied by it.
Programming in a Turing complete programming language implies that there can be 
programs that result in exponentially many and infinitely long program traces.

% \begin{proposition}[Finite Word]
% A program~\program that consists of a finite sequence of program statements, 
% where none of this statements is a conditional forwards jump nor a backwards 
% jump, produces a language that consists of a single finite word.
% \end{proposition}
% 
% \vspace{-3mm}
%\begin{proposition}[Finite Set of Words] 
% A program~\program that consists of a finite sequence of statements, where some of 
% the statements are conditional forward jumps, but \emph{none of them is a 
% backwards jump}, produces a language with a finite set of words.
% The number of words is exponential in the number of conditional forward jumps.
% \end{proposition}
% 
% \vspace{-3mm}
% \begin{proposition}[Infinite Word]
% A program~$\program$ that consists of a finite sequence of statements, 
% where at least one of them is a \emph{unconditional backwards jump} and none of them is a 
% conditional forwards jump produces a language with a infinitely large word. 
% \end{proposition}
% 
% \vspace{-3mm}
% \begin{proposition}[Infinite Set of Words]
% A program~$\program$ that consists of a finite sequence of statements, 
% where at least one of them is a \emph{conditional backwards jump}, 
% produces a language with a infinitely large set of words. 
% \end{proposition}

\section{Program Specification}
\label{concept:specification}%
\label{concept:properties}%
Since we aim at checking the correctness of programs, we need a 
formalism to specify which words are considered to be correct, that is, 
within the specification and which words violate the specification---and 
represent incorrect words~(runs).
A \emph{specification} formulates requirements as a set of 
properties~$\propertiesss \subset \properties$.
The set of all properties is denoted by~\properties.
A program can be seen as a refined form of a specification, that is, 
program and specification have different levels of abstraction.
We consider each property to be a program concern, that is, 
$\properties \subset \concerns$.
%
% A formal specification describes the set of words that are desired;
% the complement, that is a specification that describes the set of words
% that are not desired is called~\emph{falsification specificaiton}.

From the discussion of programs that are written in Turing complete 
languages, we have learned that the language~$\langua(\program)$ of a 
program can have infinitely long and exponentially many words, 
and all of them could be correct.
A means for specifying desired properties of such execution sequences 
\recap{LTL}
is Linear Temporal Logic~(LTL)~\cite{Vardi1996,GastinOddoux2001},
which extends classical logic and is considered to be one natural 
and unambiguous way of describing the temporal behavior of 
a computer program~\cite{Lamport1983}.

\subsection{Safety and Liveness}
We distinguish between safety properties and liveness 
properties~\cite{Lamport1977,MannaPnueli1992}, 
and do not discuss hyperproperties~\cite{Hyperproperties}:
%
\recap{Safety Properties}
A~\emph{safety property} specifies that something (bad) must not happen~\cite{Lamport1977}.
% Lamport~\cite{Lamport1977} gives partial correctness as an example for a safety
% property. 
Checking safety properties is equivalent to checking invariants, 
that is, we check that the (global)~invariant is always 
satisfied~(a violation never happens); assertions that always 
hold are a typical example for invariants.
The violation of safety properties is witnessed by counterexamples
of finite length~\cite{KupfermanVardi2001}.
\recap{Test Goals}
Please note that also \emph{test goals}~\cite{GargantiniHeitmeyer1999,RayadurgamHeimdahl2001,FShell,MultiGoalReachability} are 
expressible as safety properties---literature also uses the 
term \emph{never claims}~\cite{EngelsEtal1997} or \emph{trap properties}~\cite{GargantiniHeitmeyer1999}.
Tests goals can be derived based on a coverage criteria~\cite{FShell}.
%
\recap{Liveness Properties}
A~\emph{liveness property} specifies that something (good) must 
happen eventually---that is, after a finite number of steps. 
The violation of a liveness property is witnessed by a counterexample
of infinite length; checking liveness requires to prove termination. 
% To some extend, liveness checking can be performed as 
% safety checking~\cite{SchuppanBiere2006}.

% Classifying Properties: An Alternative to the Safety-Liveness Classification* 
% Recognizing safety and liveness
% Defining liveness
% Safety without Stuttering
% Secure Information Flow as a Safety Property
% Checking Safety Properties Using Induction and a SAT-Solver
% Safety and liveness from a methodological point of view
% On characterization of safety and liveness properties in temporal logic
% Sistla
% "Sometime" is sometimes "not never": on the temporal logic of programs
% Composing specifications
% Synthesizing Monitors for Safety Properties
% Model Checking of Safety Properties
% Property specification patterns for finite-state verification
% A lattice-theoretic characterization of safety and liveness
% Hyperproperties
% Towards Incrementalization of Holistic Hyperproperties
% Proving the Correctness of Multiprocess Programs

\subsection{Behavior and State}

Literature also distinguishes properties based on the extent to which 
temporal aspects are relevant. 
For example, if we say that we check the correctness regarding a 
specification, we also say that we check that there are no 
\emph{states} or \emph{behaviors} that violate the specification.
The Oxford Dictionary defines ``to behave'' as ``act or conduct 
oneself in a specified way'', whereas ``the state'' is defined 
as ``the particular condition that someone or something 
is in at a specific time.''
The model checking community uses~\cite{SharyginaEtal2004} the 
terms \emph{data property}~(data-dependent property) 
and \emph{control property}~(control-dependent property) to 
talk about state and behavior.

\recap{Control Properties}
A pure \emph{control property} only refers to the control flow, 
that is, the sequence of program operations or control locations.
The control locations in a sequence thereof must 
appear in a particular temporal order.
This corresponds to the expressiveness that is brought by the 
temporal operators of temporal logic.
\recap{Data Properties}
A pure \emph{data property} does not have a notion of temporal order:
It does not refer to any (sequence of) control locations.
It makes propositions about data locations and their values for
one point in time only.

Please note that control properties can be converted to data 
properties and vice versa~\cite{ChakiEtal2004a}. 
Also, hybrid forms of these property types are possible.
Dually, safety checking (reachability) can be expressed as 
global invariant checking~\cite{PitermanPnueliEtal2018},
and liveness checking can be performed as safety 
checking~\cite{SchuppanBiere2006}.

% some say: control property if only variables get referenced that determine
% the control flow; this definition is blurry since all safety properties
% can be encoded as reachability of control locations.
%
% literature states that control-properties are also given if only
% variables get refered to that encode status of a system component
% 
%  \cite{SharyginaEtal2004}

\section{Program Semantics and Model}
\label{sec:soundcomplete}%

After the previous section has introduced the syntactical program 
representation, 
we now discuss how we represent and model the semantics of program 
executions and their space of possible behaviors and states.

Some general terms and definitions upfront:
A proposition in the form of a phrase~$a$ is said to be~\emph{valid}
if it is true for all its possible interpretations.
The \emph{denotation function}~$\sem{a}$ provides the set of all semantically
valid interpretations of a phrase~$a$.
Two phrases~$a$ and $b$ are said to be semantically equivalent~$a \equiv b$ 
if $\sem{a} = \sem{b}$.
A proposition~$b$ is a semantic consequence of a proposition~$a$,
that is, $a \sementail b$, if~$\sem{a} \subseteq \sem{b}$.
\recap{Overapproximation}
We say that proposition~$b$ \emph{overapproximates} proposition~$a$ if
$\sem{a} \subseteq \sem{b}$.
\recap{Soundness and Completeness}
A decision procedure is called to be~\emph{sound} if only logically valid 
propositions are deduced.
A decision procedure is said to be~\emph{complete} if all logically valid
propositions can be deduced.

% formula is \emph{T-satisfiable} if there exists a structure (interpretation)
% that satisfies both the sentences of theory T and the formula,
% corresponds to $\synentails$,
% also reads as "formula is satisfiable in T"

% a formula is \emph{T-valid} if all structures that satisfy all sentences
% of T also satisfy the formula,
% corresponds to $\sementails$,
% also reads as "formula is valid in T"

% logically valid if correct for all possible interpretations,
% check using unsat: there exists no interpretation for the negation 

% $\synentail$: RHS is a propositions that can be derived from the LHS, 
% that is, RHS is provable from LHS, \emph{syntactic consequence}

% $\sementail$ RHS is true for all possible interpretations of LHS

% every valid statement is the conclusion of a formal deduction.
% A proof method is \emph{complete} if~\cite{LogicHandbook}
% from~$\model \sementail \varphi$ also follows that~$K \synentail \varphi$.

% A proof method is \emph{sound} if~\cite{LogicHandbook}
% from~$\model \synentail \varphi$ also follows that~$K \sementail \varphi$.

%soundness: 
%   reliability of the conclusion that was reached,
%   validity with the respect to the semantics,
%   preserve truth,
%   every provable proposition is true

%    every provable statement is true in all interpretations 

  % ''statement is sound if it is valid and all its premises are known to be true''

% complete:
%  every possible proposition about a system can be proven

% $A \sementail B$ if and only if $\sem{A} \subseteq \sem{B}$

% $\sem{A}$: all interpretations that make A \true

% syntactic consequence~\synentail

% semantic consequence~$A \sementail B$: B is provable from A

% $\rho \sementail \formula$ iff $\forall_{m \in \sem{\rho}} : m \sementail \formula$

% $\true \sementail \false$ is incorrect

% $A$ is semantically equivalence to~$B$, written as $A \equiv B$,
% if $\sem{A} = \sem{B}$.

\subsection{Predicate Logic}
\label{concept:predicate}%
\label{concept:predicatelogic}%
The semantics of programs can be captured in formulas in predicate 
logic~\cite{SymbolicExecution,PredicateAbstraction}---also 
known as first-order logic.
Predicate logic is defined based on a set~$\logicvariables$ of variables,
a set of logical symbols~$\logicsymbols$, 
a set of $n$-ary functions~$\logicfunctions$, with~$n\geq 0$,
a set of $m$-ary predicates~$\logicpredicates$, with~$m>0$,
and a set of rules to derive well-formed formulas~$\formulas$
in predicate logic.
We use the set of logical operators~$\logicsymbols = \{ \forall, \exists, \land, \lnot, \lor, \limplies, \lequals \}$ with their common meaning.
%We use the binary operators \emph{disjunction}~$\lor$~(or), \emph{conjunction}~$\land$~(and),
% \emph{implication}~$\limplies$~(entails), and \emph{bi-implication}~$\lequals$,
% and the unary operator \emph{negation}~$\lnot$~(not).
A binary operators~$\ast \in \logicsymbols$ on formulas forms the 
relation~$\ast: \formulas \times \formulas \rightarrow \formulas$,
a unary operator~$\star \in \logicsymbols$ forms the relation~$\star: \formulas \rightarrow \formulas$.
We use the symbols~$\formula, \varphi, \psi, \rho \in \formulas$ to denote 
separate formulas.
A \emph{predicate} asserts attributes of a set of objects;
it is a formula in predicate logic with~$n$ free variables.
\recap{Vocabulary}
The \emph{vocabulary} of a formula~$\formula$ is the set~$\vocabulary(\formula)$
of all symbols that identify variables and functions.
The set of all predicate 
formulas~$\predicates \subseteq (\formulas \cup \{ \true, \false \})$
also includes the formulas \true and \false.

\recap{$\allsat$}
Given a formula~$\formula \in \formulas$ and a sequence of 
Boolean variables~$V \in \logicvariables^*$, 
the operator~$\allsat: \formulas \times 2^\logicvariables \rightarrow \Bools^*$
returns a truth table, where each row corresponds to a truth 
assignment to the variables~$V$ that make~$\formula$ satisfiable.

\subsection{Lattices}
\label{concept:lattice}%
\newcommand{\powerlatticeof}[1]{\ensuremath{\mathsf{pw}(#1)}\xspace}%
\newcommand{\flatlatticeof}[1]{\ensuremath{\mathsf{fl}(#1)}\xspace}%
\newcommand{\maplatticeof}[2]{\ensuremath{\mathsf{ml}(#1, #2)}\xspace}%
\newcommand{\downpowerlatticeof}[1]{\ensuremath{\wp_\downarrow(#1)}\xspace}%
\newcommand{\downlatticeof}[1]{\downpowerlatticeof{#1}}%
\newcommand{\downsetsof}[1]{\ensuremath{\mathcal{I}(#1)}}%
\newcommand{\downsetof}[1]{\ensuremath{\downarrow #1}}%
\newcommand{\latticeof}[1]{\ensuremath{\dddot{#1}}}%
\newcommand{\latelems}{\ensuremath{E}\xspace}%
Lattices are one of the most fundamental structures on that 
this work builds on.
They are used, for example, to compute 
abstractions~\cite{AbstractInterpretation}.
Building program analyses based on 
lattices~\cite{Monotone,AbstractInterpretation} 
allows relying on fixed-point theorems for checking convergence in the 
state-space exploration process~\cite{Kupka1997}.

\subsubsection{Lattice}
We define a (complete) \emph{lattice}~\cite{Graetzer2011} as a 
tuple~$\lattice = (\latelems, \less, \meet, \join, \top, \bot)$, 
with a set of \emph{abstract entities}~$\latelems$
and an \emph{partial order relation}~$\less \; \subseteq \; \latelems \rightarrow \latelems$.
\recap{Inclusion Relation}
The relation~$\less$ is also called the \emph{inclusion relation}~\cite{Whitman1946},
and implies a graph that represents this relation~\cite{Birkhoff1935}.
The operator~\emph{meet} (infimum) is a relation~$\meet: (\latelems \times \latelems) \rightarrow \latelems$ that provides the \emph{greatest lower bound} for a given 
pair~$(\abstentity_1, \abstentity_2) \in \latelems \times \latelems$
of abstract entities.
The operator join (supremum) is a relation~$\join: \latelems \times \latelems \rightarrow \latelems$ that provides the \emph{least upper bound} 
for a given pair of abstract entities.
%
The \emph{bottom} entity~$\bot$ is the \emph{least} in the 
partial order relation,
that is, there exists no other entity~$\abstentity \less \bot$, with~$\abstentity \neq \bot$.
The \emph{top} entity~$\top$ is the \emph{greatest} 
in the partial order relation,
that is, there exists no other entity~$\top \less \abstentity$, with~$\abstentity \neq \top$.
%
The operators~$\meet$ and~$\join$ extend to sets naturally: The meet over
a set of abstract entities is denoted by~$\bigmeet: 2^\latelems \times \latelems$, 
and the join by~$\bigjoin: 2^\latelems \times \latelems$,
for example, $\bot = \bigmeet \latelems$ and $\top = \bigjoin \latelems$.
%
A~\emph{join semilattice} is similar to a complete lattice except 
that no meet is available for all entities in~$\latelems$.
A~\emph{meet semilattice} is similar to a complete lattice except 
that no join is available for all entities in~$\latelems$.
That is, a \emph{semilattice} either has no meet or no join for all abstract entities.
%
Partially ordered sets (\emph{posets}) can be made semilattices, 
and semilattices can be made \emph{complete} by adding 
additional abstract entities 
with special meaning~(supremum or infimum)~\cite{LatticeTheoryComputerScience}.
% For example, the poset~$(\Natsz, <)$ over the natural numbers, with their 
% total order relation~$< \; \subseteq \; \Natsz \times \Natsz$ is 
% a meet semi-lattice, because all elements have an infimum (minimum element),
% which is~$\bot = 0 \in \Natsz$.
% This meet semi-lattice can be made complete by adding an artifical supremum,
% for example, $\top = \infinite$.
%% Using an infinite element is somehow broken because this does 
%% not reflect the idea of abstraction

\subsubsection{Flat Lattice}
\label{concept:flatlattice}%
A~\emph{flat lattice}~\cite{YiHarrison1993,Graetzer2011} is a 
widely used type of lattice over a set of elements~$\latelems$.
\recap{$\flatlatticeof{E}$}
We denote such a lattice over~$\latelems$ by~$\flatlatticeof{E} = 
(\latelems, \less, \meet, \join, \top, \bot)$.
A~given pair of elements is the inclusion relation~$(e_1, e_2) \in \less$ 
if and only if the first element~$e_1 = \bot$ is the bottom element
or if the second element~$e_2 = \top$ is the top element of 
the lattice.

\subsubsection{Map Lattice}
\label{concept:maplattice}%
\newcommand{\keys}{\ensuremath{\textsf{keys}}}%
\recap{$\maplatticeof{K}{\latticeof{V}}$}
A \emph{map lattice}~$\maplatticeof{K}{\latticeof{V}} = (2^{K \rightarrow V}, \less, \meet, \join, \top, \bot)$
is a lattice of elements that are maps, that is, the elements are
functions that map from a set~$K$ of keys to a set~$V$ of values; 
the values of this map are elements of another  
lattice~$\latticeof{V} = (V, \less_V, \meet_V, \join_V, \top_V, \bot_V)$.
Such a lattice are also known as \emph{function lattice}~\cite{DuffusJonssonRival1978,BackWright1990}.
The inclusion relation~$\less$ has element~$(m_1, m_2) \in \less$ 
if and only if $\forall k \in K:  m_1(k)_\bot \less_V m_2(k)_\bot$.
\recap{$m(k)_\bot$}
In the following, we rely on the function $m(k)_\bot = m(k) \; \text{if} \; (k, \cdot) \in m \; \text{otherwise} \; \bot_V$ 
which returns the value for a given key~$k$ from a map~$m$, and the 
bottom element of the value lattice if no entry for the key is present.
The meet~$\meet$ is defined by~$\meet(m_1, m_2) = \{ (k, v_1 \meet_V v_2) \, | \, (k, v_1) \in m_1 \land v_2 = m_2(k)_\bot \}$,
the join~$\join$ is defined by $\join(m_1, m_2) = \{ (k, m_1(k)_\bot \join_V m_2(k)_\bot) \, | \, k \in \keys(m_1) \cup \keys(m_2) \}$,
the top element~$\top$ is defined by~$\top = \{ (k, \top_V) \, | \, k \in K \}$,
and the bottom element~$\bot$ is defined by~$\bot = \{ (k, \bot_V) \, | \, k \in K \}$.

\newcommand{\imagejoin}{\ensuremath{\bigjoin_\rightarrow}\xspace}%
\recap{Operator \imagejoin}
We define an \emph{image-join operator}~$\imagejoin: 2^{K \times E} \rightarrow 2^{K \rightarrow E}$:
Given a map~$M \subseteq K \times E$, with a set of keys~$K$, and 
a set of lattice elements~$E$, the operator joins all tuples~$(k, e) \in M$ 
with the same key~$k$ into one tuple with a value that aggregates 
all value elements~$e$, that is, 
$\imagejoin M = \{ \; (k, \bigjoin \, \{ e \; | \; e \in \{ (k, e) \in M \} \} ) 
    \; | \; k \in \{ k \; | \; (k, \cdot) \in M \} \; \} 
$.

\subsubsection{Powerset Lattice}
A powerset lattice that describes a Hoare powertheory~\cite{HandbookOfLogic,FergusonHughes1989,HartTsinakis2007}---%
over a given lattice~$\latticeof{E} = (\latelems, \less_E, \meet_E, \join_E, \top_E, \bot_E)$---%
is denoted by~$\powerlatticeof{\latticeof{E}} = (2^\latelems, \less, \meet, \join, \top, \bot)$,
\recap{$\powerlatticeof{\latticeof{E}}$}
where the set of elements is constituted by the set of all 
subsets~$2^\latelems$ of the set~$\latelems$.
The inclusion relation~$\less$ has the element~$(E_1, E_2) \in \less$ 
if and only if~$\forall e_1 \in E_1 \exists e_2 \in E_2: e_1 \less_E e_2$.
The join~$\join(E_1, E_2) = E_1 \cup E_2$ is the union,
and the meet~$\meet(E_1, E_2) = E_1 \cap E_2$ is the intersection
of two given sets~$E_1, E_2 \subseteq E$.
The bottom element~$\bot = \emptyset$ is the empty set,
and the top element~$\top = E$ is the set with all elements.

\subsubsection{Prefix Lattice}
It is well known~\cite{Brookes1983,WinkowskiMaggioloSchettini1987,AbadiPlotkin1993}
that a (sequential)~program can be characterized 
by a prefix-closed set of sequences program operations.
A set~$W$ of words is called \emph{prefix closed} if for each
word~$\word \in W$ also every single prefix of the word is 
included in the set~$W$.
That is, a set~$W$ is prefix closed if it is a downset regarding
a partial order of words that describes whether or not one
word is prefix of another word.
The prefix lattice describes a corresponding partial order 
of words:
%
\newcommand{\prefixlatticeof}[1]{\ensuremath{\mathsf{pr}(#1)}\xspace}%
The \emph{prefix lattice}~$\prefixlatticeof{\Sigma^\infty} = 
(\Sigma^\infty, \less, \meet, \join, \top, \bot)$ 
describes the relationship between words~$\Sigma^\infty$
over an alphabet~$\Sigma$.
\recap{$\prefixlatticeof{\Sigma^\infty}$}
A word is a sequence~$\word = \langle \sigma_1, \ldots \rangle \in \Sigma^\infty$ 
of symbols from the alphabet~$\Sigma$.
Two words are in the inclusion relation~$(\word_1, \word_2) \in \less$,
with~$\less \subseteq \Sigma^\infty \times \Sigma^\infty$,
if and only if word~$\word_1$ is prefix of word~$\word_2$.
A word~$\bar{a}$ is \emph{prefix} of a word~$\bar{b}$ if and only 
if $\bar{a} = \bar{b}$ or $\forall_{i = 1 \ldots n} b_i = a_i$,
where $a_i$ is the $i$th letter of the corresponding word,
and $n$ is the length~$|\bar{a}|$ of the word~$\bar{a}$.
The definitions of the join~(least upper bound)~$\join: 
\Sigma^\infty \times \Sigma^\infty \rightarrow \Sigma^\infty$, 
and the meet~(greatest lower bound) follow from the relation~$\less$.
The bottom symbol~$\bot$ of the lattice corresponds to the empty word~$\epsilon$.
The symbol~$\top$ is added to complete the lattice such that for
all~$\word \in \Sigma^\infty$ holds that~$(\word, \top) \in \less$.

\subsubsection{Boolean Algebra}
Any complemented distributive lattice is isomorphic to a Boolean 
algebra~\cite{Huntington1904},
which also follows from the Stone duality~\cite{Stone1936};
one example for such lattices are powerset lattices.
Lattices generalize Boolean algebras by not requiring 
complement and distributivity in the first hand.

\subsection{Abstraction}
\label{concept:abstraction}%
\label{concept:abst}%
\label{concept:sem}%
\label{concept:abstdomain}%
\label{concept:abststate}%
\newcommand{\concrete}{\ensuremath{C}\xspace}%
\newcommand{\semilattice}{\ensuremath{\mathcal{E}}\xspace}%
We reason about the states of a program on a computer
and distinguish between concrete states and abstract states.
One \emph{concrete state} represents the full state 
of a computer at one point (CPU cycle) in time---a concrete state 
can be seen as one vector of bits.
One \emph{abstract state} describes a set of concrete states---a 
set of concrete states is sometimes called \emph{region}.

\subsubsection{Abstract Domain}
The \emph{abstract domain}~\cite{CPA} defines mechanisms for 
mapping between concrete and abstract entities and for reasoning 
about the relationship between abstract entities.
The abstract domain concept we build on was introduced in 
the context of abstract interpretation~\cite{AbstractInterpretation,CousotPOPL79,FileEtal1996}
and is the foundation for several program analysis 
frameworks~\cite{Saidi2000,SchmidtSteffenSAS98,CousotProgress2001,CousotCousot2002,Monotone,CPA}.
An abstract domain~$\abstdomain = (\concrete, \semilattice, \sem{\cdot}, \abst{\cdot})$
is an algebraic structure that consists of the set of concrete 
elements~\concrete, a (semi-)lattice~$\semilattice = (\abststates, \top, \bot, \sqsubseteq, \join, \meet)$
on the set~$\abststates$ of abstract elements, a denotation 
function~$\sem{\cdot}: \abststates \rightarrow 2^\concrete$,
and an abstraction function~$\abst{\cdot}: 2^\concretes \rightarrow \abststates$.
The \emph{denotation} (concretization) function~$\sem{\cdot}: \abststates \rightarrow 2^\concretestates$
maps from an abstract state~$\abststate \in \abststates$ to a 
set~$C \subseteq \concretestates$ of concrete elements.
The denotation~$\sem{\abststate}: \abststates \rightarrow \powset{\concretes}$ 
of an abstract element~$\abststate$ is the set of all its 
possible interpretations---as known from denotational semantics~\cite{HandbookOfLogic}.
The \emph{abstraction} function~$\abst{\cdot}: 2^\concretestates \rightarrow \abststates$
maps from a set of concrete elements to an abstract state, that is, 
it is a surjection that provides a \emph{symbolic representation}.
%
The abstraction~$\abst{\concretes_k}$ of a set of concrete 
elements~$\concretes_k \subseteq \concretes$ results in an 
abstract element~$\abststate$, with~$\sem{\abststate} = \concretes_k$. 
Please note that constructing a symbolic~(abstract) representation 
does not imply any loss of information.

Two elements are called \emph{semantically equal}, that is, 
$\abststate_1 \equiv \abststate_2$, if and only 
if~$\sem{\abststate_1} = \sem{\abststate_2}$ in the same universe.
One element \emph{semantically implies} another element,
that is, $\abststate_1 \sementail \abststate_2$, if and only
if~$\sem{\abststate_1} \subseteq \sem{\abststate_2}$.

\subsubsection{Widening}
The term abstraction is typically associated with a loss 
\recap{Abstraction Precision}
of information, that is, the number of interpretation 
of a given entity is increased.
We reflect this in the abstraction function~$\abst{\cdot}^\precision: \abststates \rightarrow \abststates$
\emph{with widening}.
The widening is performed based on a given \emph{abstraction precision}~$\precision \in \precisions$~\cite{NayakLevy1995},
which defines the set of details (facts) to keep or to discard.
The result of a widening~$\abststate' = \abst{\abststate}^\precision$ 
in a new abstract element~$\abststate'$ 
with~$\sem{\abststate} \subseteq \sem{\abststate'}$. 

\subsubsection{Composite Domain}
A list of abstract domains~$\abstdomain_1, \ldots, \abstdomain_n$ can be 
combined~\cite{CPA} to form a~\emph{composite domain}~$\abstdomain_\times$. 
A composite domain operates on~\emph{composite elements} $E_\times \subseteq E_1 \times \ldots \times E_n$,
which are elements of a \emph{product lattice}, and 
form tuples of abstract elements from the component domains~\cite{CPA}.  

% \newcommand{\powerdomainof}[1]{\ensuremath{\wp(#1)}\xspace}%
% \newcommand{\downpowerdomainof}[1]{\ensuremath{\wp_\downarrow(#1)}}%
% \newcommand{\powerdomain}{\ensuremath{\hat{\abstdomain}}}%

% Relationship of abstract domain, lattice, and the operations of the program analysis
% (what does manipulating abstract states mean with respect to the lattices?)

% In which cases can we get sound results
% while tracking different variables with different abstract domains?

\subsection{Concrete and Abstract Semantics}
\label{concept:sp}%
\label{concept:post}%
\label{concept:spost}%
We define the semantics of a program operationally
and rely on the formalization that is provided with predicate
transformers~\cite{PredicateTransformers}---as used in predicate
abstraction~\cite{PredicateAbstraction}.
One formula~$\formula \in \formulas$ denotes a set~$\sem{\formula}$
of concrete program states.
\recap{Strongest Postcondition}
The \emph{strongest postcondition} is an operator~$\spost: \formulas \times \ops \rightarrow \formulas$.
That is, the result of a call $\spost_{\op}(\formula)$, 
also written as~$\spost(\formula, \op)$, 
results in a new formula~$\formula'$ that satisfies the 
Hoare triple~$\{\formula\} \; \op \; \{\formula'\}$~\cite{Hoare1969}.
The operator naturally extends to sequences of program 
operations such as~$\sequence = \vstart \op_1, \ldots, \op_n \vend \in \opseqs$,
that is, $\spost_\sequence(\formula) = \spost(\op_n,(\ldots, (\spost(op_1, \formula))$.

Since we model the state space of a program based on an abstract 
domain~$\abstdomain = (\concrete, \semilattice, \sem{\cdot}, \abst{\cdot})$,
we use the term~\emph{abstract state} for an abstract element
that describes a set of concrete (program) states.
An abstract state~$\abststate \in \abststates$ is an element in 
the corresponding lattice~$\semilattice$ of abstract states~$\abststates$.
The set~$\concrete$ corresponds to the set of \emph{concrete states}.
%
We overload the strongest postcondition operator to operate on
abstract states~$\spost: \abststates \times \ops \rightarrow \abststates$,
and on concrete states~$\spost: \concrete \times \ops \rightarrow 2^\concrete$.

Each concrete state~$c \in \concstates$ is a map of data locations~$\datalocs$
to corresponding data values with the respective type---we restrict 
the discussion to integers for now.
We assume that each operation is atomic regarding its execution 
on a computer. The current status of a computer can be observed 
in discrete points in time.

% we define the semantics of a program based on trace semantics~\cite{Cousot2001}.

% trace semantics (better for matching based on automata!!)
% \cite{Cousot2001}

% see https://www.di.ens.fr/~cousot/COUSOTpapers/publications.www/Cousot-LNCS2000-sv-sb.pdf


\subsection{Transition Systems}
\label{concept:transsystem}%
\label{concept:kripke}%
\label{concept:arg}%
The semantics of a program, with all its states and behaviors, can 
be captured in a transition system, for example, a Kripke 
structure~\cite{Browne1986,ClarkeEtal1986}.
A software model-checking procedure creates a reachability graph 
to prove a safety property, 
%
A control-flow automaton~\cfa, in contrast, describes a program on 
a syntactical level, that is, it has a language~$\langua(\cfa)$ that 
consists of all syntactically well-formed program control paths. 

\subsubsection{Abstract Reachability Graph}
\label{concept:arg}%
An~\emph{abstract reachability graph}~(ARG)
is a graph~$\reachgraph = (R, \abststate_0, \transabs{}{})$,
with a set of reached abstract states~$R \subseteq \abststates$,
an initial abstract state~$e_0 \in R$,
and an abstract transfer relation~$\transabs{}{} \subseteq \abststates \times \abststates$.
That is, each node corresponds to an abstract state~$e \in R$, 
and an edge between two nodes~$e$ and $e'$ represents the transition 
$(e, e') \in \transabs{}{}$ between two abstract states---which 
we also write as~$e \transabs{}{} e'$.
The ARG is implicitly parameterized with an abstract domain~$\abstdomain$
that provides the mapping between abstract states and concrete states.
The \emph{size of an abstract reachability graph}---also referred 
to as the \emph{size of the abstract model}, or the \emph{size of 
the abstract state space}---is the number of abstract states~$|R|$.
%
We called an abstract reachability graph to be \emph{labeled}
if each transition $(e, e') \in \transabs{}{}$ between abstract 
states is labeled with a program operation~$\op \in \ops$ of
a corresponding control flow transition~$g = (\location, \op, \location') \in \controlflows$.
The labeling is made explicit by the labeled transfer
relation~$\transabs{\ops}{} \subseteq \abststates \times \ops \times \abststates$.

Compared to a Kripke structure~\cite{KupfermanEtal2000,Browne1986,ClarkeEtal1986}, 
an ARG does not have a notion of state labeling, but such a 
labeling can be performed, such that the ARG is \emph{lifted}
to become a full or partial~\cite{Wehrheim2008} Kripke 
structure~\cite{BrunsGodefroid1999,Wehrheim2008}.

% \section{Composition}
% 
% \cite{KestenPnueli1998}
% Different types of composition
% synchronous/asynchronous
% introduce a compositional framework for shared variables
% 
% \emph{synchronous parallel composition}
% 
% one application example: spc with a~\emph{tester} for the negation of the specification
% \cite{KestenPnueli1998}
% 
% equivalent  to the composition of CPAs, 
% where one of the specs represents the negation of the specification

\subsubsection{Program Path}
\recap{Abstract Program Path}%
An~\emph{abstract program path} is a sequence 
$\abstpath = \vstart e_0, \ldots, e_n \vend \in \abststates^\infty$ 
of abstract states that starts in the initial state~$e_0 \in \abststates$, 
and is well-formed regarding the transfer relation~$\transabs{}{}$
of the corresponding abstract reachability graph; 
we also write it as with~$e_0 \transabs{}{} \ldots \transabs{}{} e_{n}$.
%
\recap{Concrete Program Path}
One abstract program path represents a set of concrete program 
paths~$\sem{e_0} \transabs{}{} \ldots \transabs{}{} \sem{e_{n}}$.
A \emph{concrete program path} is a path~$c_0 \trans{}\ldots\trans{} c_n$, with~$c_i \in \sem{e_i}$.
An abstract program path is \emph{feasible} if each abstract state along
the path has a concrete counterpart, 
that is, $\forall_{i \in [ 0, n ]} \exists \: c_i \in \sem{e_i}$,
otherwise it is called \emph{infeasible}.
A concrete program path is also called a~\emph{test vector}.

\subsubsection{Inductive Invariants}
Given a transition system in the form of an ARG~$(R, e_0, \transabs{}{})$.
A formula~$\formula \in \formulas$ is an \emph{inductive invariant} for this transition 
system if (1)~then invariant holds in the initial state~$e_0$, 
that is, $\sem{e_0} \subseteq \sem{\formula}$,
and (2)~it holds for every state~$e'$ that is transitively reachable
on the transition relation~\cite{Floyd1967,PadonEtal2016}, 
that is, $\sem{e'} \subseteq \sem{\formula}$.
A sequence of abstract states~$\abstpath = \vstart e_1, \ldots, e_n \vend$
satisfies invariant~$\formula$ if and only 
if~$\forall_{e_i \in \abstpath} \sem{e_i} \subseteq \sem{\formula}$.

% \subsection{Bisimulation and Refinement}

% defined based on transition systems, which model the semantics,
% also defined for automata: \cite{DamsLakhnechSteffen2002}


% important:
% \cite{SchmidtSteffen1998}

% The correctness of abstractions is proven using simulation relations

% \url{https://en.wikipedia.org/wiki/Bisimulation}

% Super-Abstract: Software Art and a Redefinition of Abstraction

% The transfer relation defines the semantics

% \begin{figure}[tp]
% \center
% \includegraphics[height=50mm]{figures/concrete-abstract-rel.pdf}
% \caption{Relationship between concrete and abstract states.}
% \label{fig:concabstrel}
% \end{figure}

% \ref{fig:concabstrel}

% bisimulation equivalences
% \cite{GlabbeekGoltz1990}

% relationship to trace semantics!

% behaviours of a program as a set of traces

% fixed point iteration until the set covers,
% see the work of Cousout,
% abstraction
% % Constructive design of a hierarchy of semantics of a transition system by abstract interpretation.

\section{Model Checking Programs}

Software verification is considered a grand challenge of computer science~\cite{grand-challenge}.
Several different approaches exist to verify the correctness 
of a program concerning a given specification.
We choose software model checking for this purpose.
\emph{Model checking} is an automatic, algorithmic, and 
exhaustive analysis of the states and behaviors of systems that 
can be described by state-transition systems~\cite{Handbook}.
Given a system~$S$ and a specification~$\varphi$, a model checker constructs a 
model~$K$ that overapproximates all possible states and behaviors of~$S$ and 
checks whether this model satisfies the specification~$\varphi$ or not, 
that is, $K \sementail \varphi$, where the symbol~$\sementail$ represents 
the semantic entailment.
\recap{Software Model Checker}
A \emph{software model checker} takes as input a 
program~\program (the system to verify) 
and a specification and outputs whether this specification is 
satisfied or not---in an algorithmic, automatic, and exhaustive fashion.
%
% modelling to prove statements (properties) about systems, algorithmically
%
% temporal properties (behaviour of a system over time)
%
% check if a finite-state transition structure~$\kripke$ is a model of a temporal 
% property (expressed in a temporal property).
%

\subsection{Problem Characterization}
\label{concept:explosions}

The applicability of model checking faces theoretical 
and practical limitations. 
First and foremost, Gödel's incompleteness theorem~\cite{Goedel} 
states that there cannot be a complete and sound solution for 
all possible model checking problems~(verification tasks).
% halting problem, Rice's theorem
In practice, we face the \emph{state space explosion problem}, 
which describes the fact that the size---the number of 
states and transitions---of a Kripke structure 
can be exponential several times, regarding different factors.
Each factor represents a sub-problem with high (exponential) costs on its own.

\recap{Control Explosion}
First, there is the \emph{path explosion problem} 
or \emph{control explosion problem}, 
that is, with each branching in the 
control flow, the size of the state-space potentially doubles and is therefore 
exponential in the number of branchings---there can be exponentially 
many words in the language~$\langua(\program)$ of the program~$\program$.

\recap{Unwinding Explosion}
The next dimension is the \emph{unwinding explosion problem} 
that can result in infinitely long words in the 
language~$\langua(\program)$ of the program, 
which arise from unwinding loops and recursion.
\emph{Loop invariants}~\cite{KovacsVoronkov2009,LoopInvariantsSurvey} 
are needed to construct a 
finite abstraction of this possibly infinite behavior.
In the case of liveness properties, also termination has to be proven.

\recap{Data Explosion}
Another dimension, the \emph{data explosion problem}, arises from the data 
in the system's memory. Given a system with~$|\datalocs| = n$ data locations, 
each data location is mapped to a domain $D$; the domain defines the number
of different abstract representations of different values for a data location.
The number~$|\concstates|$ of concrete states raises therefore exponential in the number
of data locations, where the factors are determined by the domains: $D_1 \times \ldots \times D_n$.
Please note that also costs of some decision procedures that are 
used for symbolic state-space representation can be quadratic or 
exponential~\cite{AllSmt} in the number of variables regarding time or space.

\recap{Interleaving Explosion}
The next dimension, the \emph{interleaving explosion problem}, arises from
all possible interleavings of code fragments (components, processes, or threads)
in the context of the analysis of concurrent systems or compositional reasoning.
The number of states in the Kripke structure can be exponential 
in the number of processes~\cite{PeledEtal2018} 
or the number of components~\cite{GiannakopoulouEtal2018} 
to interleave.

Another dimension, the \emph{configuration explosion problem}, 
is defined based on 
\recap{Configuration Explosion}
the different compile-time or run-time configurations that 
a program can have~\cite{RheinEtal2016,SPLBook}.
The number of variants a system can have is exponential in 
the number of configuration options.

\subsection{Counterexample-Guided Abstraction Refinement}
\label{concept:CEGAR}
\recap{Abstraction}
The most effective approach to cope with the state-space explosion 
is abstraction, that is, to remove~(abstract from) all details 
of the system that are irrelevant for the reasoning task at hand.
Or dually, model only those details that are relevant to solve the task.
\recap{Abstraction Precision}
The set of details of a system to model is called 
the \emph{abstraction precision}~\cite{NayakLevy1995,CPAplus}, 
which can be, for example, a set of predicates, or a set of data locations.

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[node distance=8mm, scale=0.8, transform shape]

\node[conceptstate] at (0,0)   (checking)          {$\textsf{Model Checking}$};
\node[conceptstate] at (4.3,-1.4)  (feasibility)             {$\textsf{Feasibility Check}$};
\node[conceptstate] at (4.3,1.4)   (refinement)          {$\textsf{Precision Refinement}$};
\node[inputstate,anchor=east] at (-3.5,0.6)   (program)      {$\textsf{Program}$};
\node[inputstate,anchor=east] at (-3.5,-0.6)   (spec)     {$\textsf{Specification}$};
\node[] at (0,-1.5)   (true)          {$\textsf{\textbf{TRUE}}$};
\node[] at (8.2,-1.5)   (false)          {$\textsf{\textbf{FALSE}}$};
\node[] at (-2.7,0)   (start)          {};

\path[ctrans] (start) edge [anchor=center,above] node  {$\precision_0 = \emptyset$} (checking);
\path[ctrans] (feasibility) edge [anchor=center,right] node  {$\controlpath$ infeasible} (refinement);
\path[ctrans] (checking) edge [anchor=center,above right] node  {$\controlpath = \langle l_0, \ldots \rangle$} (feasibility);
\path[ctrans] (refinement) edge [anchor=center,above] node  {$\precision'$} (checking);
\path[ctrans] (checking) edge [anchor=center,above] node  {} (true);
\path[ctrans] (feasibility) edge [anchor=center,below] node  {$\controlpath$ feasible} (false);

\node[] at (-2.5,0.6)   (programin)      {};
\node[] at (-2.5,-0.6)   (specin)      {};

\path[ctrans] (spec) edge [anchor=center,below] node  {} (specin);
\path[ctrans] (program) edge [anchor=center,below] node  {} (programin);

\draw [draw=gray!70] (-3,2.5) rectangle (9.5,-2.5); 

\end{tikzpicture}
\end{center}
\caption{Counterexample-Guided Abstraction Refinement (CEGAR)}
\label{fig:cegar}
\end{figure}

The most prominent approach to derive an abstract model that is 
sufficiently precise to prove that a program adheres to 
a given specification is
\emph{counterexample-guided abstraction refinement}~(CEGAR)~\cite{CEGAR}.
A scheme of CEGAR is illustrated in Fig.~\ref{fig:cegar}.
The abstraction process starts with an empty abstraction 
precision~$\precision_0 = \emptyset$, which is used to construct a first
abstract model~(abstract reachability graph) of the program.
The abstract model is then checked for abstract states that violate the 
specification. 
The program is safe if no violating state is found because 
the model checking procedure ensured that the abstract model 
overapproximates all possible states and behaviors that the 
concrete system can have. 
In case a violating state is found, a counterexample is constructed
\recap{Spurious Counterexamples}
as a witness for the violation; for safety properties, such a counterexample
is a finite program path~$\controlpath = \vstart \location_0, \ldots \vend$~\cite{KupfermanVardi1999}.
This path might be infeasible in the concrete program, 
that is, $\spost_{\controlpath}(\true) \equiv \false$,
and was only reachable in the abstract model due to a lack of precision;
we call such a counterexample \emph{spurious}.
\recap{Precision Refinement}
To eliminate spurious counterexamples, and to prove the absence of violations,
the abstraction precision---and with it, the abstract model---has 
to be refined. 
Additional details to model are identified based on the counterexample
and added to a new abstraction precision~$\precision'$ such
that it does not re-appear in the next iteration of the CEGAR loop.
Different techniques are available to identify the details to rule out a 
spurious counterexample, for example, Craig interpolation~\cite{Craig}.

\subsection{Craig Interpolation}
\label{sec:concept:craigitp}%
\label{sec:craigitp}%
\label{concept:craig}%
We use Craig interpolation~\cite{Craig,McMillanCraig} to 
derive precision refinements from spurious counterexamples. 
It is a technique to get a (more) abstract explanation~$\interpolant$ 
for the unsatisfiability of a formula~$\formula$ in predicate logic 
and helps to localize different facts to track alongside a 
counterexample~\cite{AbstractionsFromProofs}.

We use McMillans formulization~\cite{McMillanCraig} of the 
Craig interpolation theorem~\cite{Craig}:
Given a formula~$\formula \equiv \formula^- \land \formula^+$, a formula~$\interpolant$ 
is a Craig interpolant if and only if
\begin{equation*}
\begin{split}
                & \formula^- \land \formula^+ \; \mathit{unsat} \\
\textrm{and} \; & \formula^- \lentails \interpolant \\
\textrm{and} \; & \interpolant \land \formula^+ \; \mathit{unsat} \\
\textrm{and} \; & \vocabulary(\interpolant) \subseteq \vocabulary(\formula^-) \cap \vocabulary(\formula^+) \textrm{.}
\end{split}
\end{equation*}
A Craig interpolant can be obtained in polynomial time~\cite{HandbookInterpolation}
from the proof of an SMT solver if the background theories 
have the interpolation property.

\subsection{Predicate Abstraction}
\label{concept:predicateabstraction}%

Predicate abstraction~\cite{PredicateAbstraction} is an approach 
to summarize~(abstract or widen) a given formula~$\formula \in \formulas$ 
in predicate logic based on a set of 
predicates~$\precision \subset \predicates$. 
It is an essential~\cite{AllSmt,SLAMacm,BLAST,LBE} means to derive 
a finite abstract model of a program.
The formula that should be summarized by predicate abstraction 
represents a set~$C_\varphi = \sem{\varphi}$ of concrete program states.
A program analysis typically conducts such an abstraction at specific 
points~\cite{ABE} in the control flow---the \emph{abstraction locations}, 
for example, loop heads~\cite{LBE,ABE}.
The resulting abstraction is a Boolean combination of the given 
set of predicates~\precision, that is, it is an abstraction with 
widening~$\abst{\cdot}: \formulas \times 2^\predicates \rightarrow \formulas$,
which we also write 
as~$\abst{\cdot}^\precision: \formulas \rightarrow \formulas$.
We distinguish between Boolean predicate abstraction and Cartesian 
predicate abstraction~\cite{BooleanCartesian,LBE}:

\subsubsection{Boolean Predicate Abstraction}
A \emph{Boolean predicate abstraction}~$\abst{\formula}^\precision_\mathbb{B}$ 
of a given formula~$\formula \in \formulas$ is 
the \emph{strongest} Boolean combination~$\abstformula \in \formulas$ of 
predicates~$\precision \subset \predicates$ that is entailed by \formula, 
that is, $\formula \lentails \abstformula$~\cite{AllSmt}.  
The resulting formula~$\abstformula$ represents a set of 
concrete states such that~$\sem{\varphi} \subseteq \sem{\abstformula}$.

The predicates~$\precision$ are ordered (are assigned an index), 
which results in the list~$\bar{\predicate} = \vstart \predicate_1, \ldots, \predicate_n \vend \in  \predicates^*$ 
of predicates.
We introduce a propositional variable~$v_i \in \formulas$ and 
get~$\bar{v} = \vstart v_1, \ldots, v_n \vend \in \formulas^*$. 
We solve the following \allsat~\cite{AllSmt} problem, 
which results in a truth table~$R \subseteq \Bools^{|\predicates|}$ with at most~$2^{|\precision|}$ entries:
%
$$R = \allsat(\formula \land \Bland_{i \in 1..|\bar{\predicate}|} v_i \lequals \predicate_i, \bar{v})$$

\noindent
A row in the result table~$R$ is a tuple~$\bar{r} = \vstart r_1, \ldots, r_n \vend \in \Bools^{|\precision|}$. 
For each row~$\bar{r} \in R$ we conjunct all predicates for that the propositional
variable~$v_i$ was evaluated to \true. 
The resulting abstraction formula~$\abstformula$ is the disjunction of 
all these conjunctions:
%
$$\abstformula = \bigvee_{ \bar{r} \in R} \Bland_{\predicate_i \in \bar{\predicate}} \{ \predicate_i \: | \: r_i \equiv \true \}$$

The \allsat procedure is implemented on top of an incremental SMT solver.
A new blocking clause is pushed after each satisfying assignment.
The result is typically~\cite{AllSmt} stored in a BDD
to arrive at a compact representation and allow for fast coverage checks. 

\begin{example}
Given a formula~$\formula \equiv 
x = 2 
\land 
    ((b = x \land a > 0 \land i = 64 )
    \lor (b = x-1 \land i>128 \land a = 0) 
    \lor (i=64))$ 
to abstract using Boolean predicate abstraction with the list of 
predicates~$\bar{\predicate} = \vstart \predicate_1, \predicate_2, \predicate_3 \vend = \vstart b = 1, x = 2, i \leq 90 \vend$.
We introduce a list of propositional variables~$\bar{v} = \vstart v_1, v_2, v_3 \vend$,
where each of them has a one-to-one correspondence to the 
predicates in~$\bar{\predicate}$.
The \allsat call returns the assignments~%
$R = \{ \vstart 0, 1, 1 \vend, \vstart 1, 1, 0 \vend, \vstart 1, 1, 1 \vend \}$,
which results in the Boolean predicate 
abstraction~$\predicate_2 \land (\predicate_1 \lor \predicate_3)$.
\label{ex:booleanabst}
\end{example}

\subsubsection{Cartesian Predicate Abstraction}
Another approach for predicate abstraction is 
\emph{Cartesian predicate abstraction}~$\abst{\formula}^\precision_\mathbb{C}$ 
of a given formula~$\formula \in \formulas$.
It is the conjunction~$\abstformula \in \formulas$ of 
all predicates~$\in \precision$ that entail~$\formula$, that is,
the abstraction~$\abstformula$ results from:
%
$$\abstformula = \Bland_{\predicate_i \in \precision} \{ \predicate_i \: | \: \formula \lentails \predicate_i \}.$$

\noindent
This approach does not take dependencies between predicates into 
account and results in coarse-grained abstractions.
%
\nopagebreak[4]
%
\begin{example}
Given the formula~$\formula$ and the abstraction precision~$\precision$ 
from Example~\ref{ex:booleanabst}, 
the Cartesian predicate abstraction~$\abst{\formula}^\precision_\mathbb{C}$
results in the formula~$x = 2$.
\end{example}

% see the papers:
%    'property preserving abstractions for the verification of concurrent systems'
%  and 'model checking and abstraction'


% \subsubsection{Block Encoding Strategies}

% As in LBE/ABE

% if the code of that is relevant for a property is within a block: no refinement needed
% 
% LBE was designed to encode multiple operations into one block
% that is then sent to a SMT solver. 
% Explosion of the state space reduced

% The largest formulas in software model checking with CEGAR apear 
% when checking the feasibility of counterexamples where
% the full program path (starting from the entry location)
% gets checked.

% In LBA/ABE some infeasible counterexample can
% be excluded by checking the feasibility of blocks (conjunction
% of abstraction formula and block formula)
%
% In cases where infeasible counterexamples can already be eliminated
% with the SAT check for the block, we can safe the time
% checking the full program path of the counterexample. 

% The costs of checking SMT formulas can
% be decreased by applying slicing techniques
% that remove irrelevant variables. 
% (implemented in SMT interplol, check this!)

% Paper: "Small Formulas for Large Programs: On-line Constraint Simplification in Scalable Static Analysis"

\section{Configurable Program Analysis}
\label{concept:cpa}%

Configurable program analysis (CPA)~\cite{CPA,CPAplus} is a concept, 
formalism, and framework~\cite{CPAchecker} for formalizing and 
implementing program analyses.
It provides the foundation to combine techniques from different 
directions of research for reasoning about programs, for example, 
combinations of techniques from abstract interpretation~\cite{AbstractInterpretation}, 
data-flow analysis~\cite{Monotone}, 
symbolic execution~\cite{SymbolicExecution},
and techniques from model checking~\cite{ClarkeBook,Handbook}.
% Tools that were build based on this framework have shown remarkable 
% results in different editions of the International Competition 
% on Software Verification~\cite{SVCOMP}.

The framework was first provided within the tool~\blast~\cite{BLAST}
\recap{\cpachecker}
and was further refined and extended in 
the tool~\cpachecker~\cite{CPAchecker}, 
on which our implementation is based.
\important
We slightly modify different operators of the framework, for example, 
by adding some operators, adding parameters to existing operators, 
or remove some parameters if they are not relevant to present 
the contributions of this work. 
We indicate the modifications where appropriate.

Please note that we build on configurable program analysis~\emph{with 
dynamic precision adjustment}~\cite{CPAplus}: Different operators 
and algorithms are extended with an abstraction precision. 
\recap{Abstraction Precision}
An \emph{abstraction precision}~$\precision \in \precisions$ is a 
set of program facts to track, and determines the level of abstraction 
of the abstract model to construct; 
the set of all abstraction precisions is denoted by~$\precisions$. 
An elaborated formal definition of abstraction precisions
is provided in Sect.~\ref{concept:prec}.

\recap{Verification Engine}
We use the term~\emph{verification engine} to denote all components
of a verification tool that contribute to the verification process.
The set of components includes an SMT solver, a BDD library, different
algorithms that wrap the reachability algorithm, for example,
a CEGAR loop~\cite{CEGAR}.

\subsection{CPA Algorithm}
\label{concept:cpaalg}%
\label{sec:cpaalg}%

The \emph{CPA Algorithm}~\cite{CPA,CPAplus,ApelEtal2016} is the 
heart of the model-checking procedure that we use. 
\recap{$\wait$ and $\reached$}
It is a reachability (semi-)algorithm that operates based on a 
worklist called~$\wait$, which is a subset of the set of abstract 
states~$\reached$ that is considered reached at a given point in time.
The algorithm starts the state space exploration starting from 
an initial worklist~$\wait = W_0$ of abstract states and a set 
of initially reached states~$\reached = R_0$, and terminates 
either if the worklist is empty, that is~$\wait = \emptyset$, 
or if a target state has been found.
\recap{Target State}
A \emph{target state} is an abstract state whose absence or 
presence---depending on the type of property to check---has to 
be witnessed by the analysis.
All operators, except the operator~$\chooseop$, that are used within 
the CPA algorithm, are defined within the CPA~$\cpa$---which is 
an implicit parameter of the algorithm.
\recap{Operator $\chooseop$}
The operator~$\chooseop$ determines the state space traversal 
strategy, that is, given the set of frontier states~$\wait$, 
which state to compute successors for next. 
The CPA algorithm is typically wrapped by another algorithm, 
for example, a CEGAR loop.
The pairing of abstract states with an abstraction precision 
was introduced to allow for lazy abstraction~\cite{LazyAbstraction} 
and dynamic precision adjustment~\cite{CPAplus}.

\begin{algorithm}[t]
\begin{small}
\caption{\textbf{ }$\textsf{CPAalg}_\cpa(R_0, W_0)$, adopted from \cite{CPA,CPAplus}}
\label{alg:cpa}
\begin{algorithmic}[1]
\vspace{1mm}
\INPUT               a CPA $\cpa = (D, \transabs{}{}, \mergeop, \stopop, \precop, \targetop)$,\\
\hspace{2.6mm}       a set~$R_0 \subseteq E \times \precisions$ of abstract
                     states with precision,\\
\hspace{2.6mm}       a subset~$W_0 \subseteq R_0$ of frontier abstract 
                     states with precision,\\
\hspace{2.6mm}       where $E$ denotes the elements of the lattice of $D$
\vspace{1mm}
\OUTPUT              reached abstract states with precision,\\ 
\hspace{2.6mm}       remaining frontier abstract states with precision
\vspace{1mm}
\VARDECL             a set $\reached \subseteq E \times \precisions$,
                     a set $\wait \subseteq E \times \precisions$
\vspace{1mm}
\STATE $\reached := R_0$; $\wait := W_0$
\vspace{1mm}
\WHILE {$\wait \neq \emptyset$}
    \STATE $(e, \precision) := \popop(\wait)$
\vspace{1mm}
    \FOR{\textbf{ each} $e'$ with $e \transabs{}{} (e', \precision)$}
        \STATE $(\hat{e}, \hat{\precision}) := \precop(e', \precision, \reached)$
\vspace{1mm}
        \FOR{\textbf{ each} $(e'', \precision'') \in \reached$}
            \STATE $e_\mathit{new} := \mergeop(\hat{e}, e'', \hat{\precision})$
\vspace{1mm}
            \IF {$e_\mathit{new} \neq e''$}
                \STATE $\wait    := \big(\wait \cup \{(e_\mathit{new},\hat{\precision})\}\big) \setminus \{(e'', \precision'')\}$
                \STATE $\reached := \big(\reached \cup \{(e_\mathit{new}, \hat{\precision})\}\big) \setminus \{(e'', \precision'')\}$
            \ENDIF
        \ENDFOR
\vspace{1mm}
    \IF {$\lnot~\mathord{\stopop}(\hat{e}, \{e ~|~ (e, \cdot) \in \reached\})$} 
        \STATE $\wait := \wait \cup \{(\hat{e}, \hat{\precision})\}$
        \STATE $\reached := \reached \cup \{(\hat{e}, \hat{\precision})\}$
\vspace{1mm}
        \IF {$\targetop(\hat{e}) \neq \emptyset$}
            \STATE {\textbf{ return }} $(\reached, \wait)$
        \ENDIF
    \ENDIF
  \ENDFOR
\ENDWHILE
\vspace{1mm}
\STATE {\textbf{ return }} $(\reached, \emptyset)$
\end{algorithmic}
\end{small}
\end{algorithm}

\subsection{CPA}

The central building block of the CPA framework is the \emph{configurable 
program analysis}~(CPA) which defines, for example, how the 
concrete states and behaviors of the program under analysis 
are abstracted, to which extend information from different 
states is combined, and provide means to check whether a 
fixed-point has been reached or not.

A \emph{configurable program analysis}~(CPA) with dynamic precision 
adjustment~\cite{CPAplus} is formalized as a 
tuple~$\cpa = (\abstdomain, \transabs{}{}, \mergeop, 
\stopop, \precop, \targetop)$ of analysis components (operators):

\begin{cpaoperator}{Abstract Domain~$\abstdomain$}
The abstract domain~$\abstdomain = (\concrete, \semilattice, \sem{\cdot}, \abst{\cdot})$ 
defines the mapping between sets of concrete states and abstract states.
The set of concrete elements~\concrete corresponds to the 
concrete states; the set of abstract elements~$\abststates$ 
of the lattice~$\semilattice$ corresponds to the abstract states.
See~Sect.~\ref{concept:abstdomain} for detailed definitions 
and discussions.
\end{cpaoperator}

\begin{component}{Transfer Relation~$\transabs{}{}$}
The \emph{transfer relation}~$\transabs{}{} \subseteq \abststates \times \abststates \times \precisions$%
---sometimes called \emph{accessibility relation}---defines the 
predecessor--successor relation of abstract states, that is, it 
is the central component that defines the shape of the abstract 
reachability graph of the program to analyze.
The relation is total and must overapproximate the reachable 
states to not miss potential specification violations.
Please note that the general notion of a CPA is independent of 
the control-flow automaton of the program~(or system) to analyze.
For analyses that encode the semantics of a control-flow automaton,
the \emph{labeled transfer relation}~$\transabs{g}{} \subseteq 
    \abststates \times \controlflows \times \abststates \times \precisions$ 
has been introduced~\cite{CPA}, which defines the set of successor
states based on a given control-flow transition~$g \in \controlflows$.
For a forwards analysis, the strongest postcondition~\spost is
used to compute the set of successor states for a given
abstract state---see Sect.~\ref{concept:sp}.
\end{component}

\begin{operator}{$\stopop$}
\label{concept:stopsep}%
\label{concept:stopjoin}%
The \emph{coverage check} operator~$\stopop: \abststates \times 2^\abststates \rightarrow \Bools$
determines~\cite{CPA} if a given abstract state is already covered sufficiently 
by the current set of reached states.
A call~$\stopop(\abststate, R)$ gets as argument the abstract
state~$\abststate \in \abststates$ to check coverage for, the
set of reached states~$R$ that might already cover the newly reached state.
To be sound---for example, for model checking---we require 
that~$\sem{\abststate} \subseteq \bigcup_{r \in R} \sem{r}$.
Literature defines two standard stop operators~\cite{CPA}:
$\stopsepop(\abststate, R) = (\exists r \in R: e \less r)$
and $\stopjoinop(\abststate, R) = (e \less \bigcup_{r \in R} r)$.
\end{operator}

\begin{operator}{$\mergeop$}
\label{concept:mergejoin}%
\label{concept:mergesep}%
The \emph{merge operator}~$\mergeop: \abststates \times \abststates \times \precisions \rightarrow \abststates$
determines how and to which extent information of a pair of abstract states should 
get combined to a new (more abstract) abstract state.
It controls if two abstract states should be combined 
or if they should be explored separately and separate the state space. 
The default is to separate two different abstract states always.
The semantics of the operator also follow from its usage in the CPA algorithm:
Given a call~$\mergeop(\abststate, \reachedstate, \precision)$, the result is computed by
widening the second argument~$\reachedstate$ based on the first 
argument~$\abststate$---that is, the operator is not commutative.
To be sound, the operator must ensure that~$\sem{\reachedstate} \subseteq \sem{\mergeop(\abststate,\reachedstate, \precision)}$.

\recap{$\mergejoinop$}
In a path-insensitive data-flow analysis, the merge operator combines
two abstract states based on the join~$\join$ of the lattice that is defined
along with the abstract domain. This behavior is implemented in the 
operator~$\mergejoinop(\abststate, \reachedstate, \precision) = (\abststate \join \reachedstate)$~\cite{CPA}.
%
\recap{$\mergesepop$}
Another merge operator is~$\mergesepop$ that always keeps 
information of two abstract states separated:
$\mergesepop(\abststate, \reachedstate, \precision) = \reachedstate$, which
means that the second argument is not widened~\cite{CPA}.
\end{operator}

\begin{operator}{$\precop$}
The \emph{precision adjustment operator}~$\precop: \abststates \times \precisions \times 2^{\abststates \times \precisions} \rightarrow \abststates \times \precisions$~\cite{CPAplus}
can provide a new abstract state with an adjusted abstraction precision.
Given a call~$\precop(\abststate,\precision,R)$, the operators 
returns a pair~$(\abststate', \precision')$, 
with~$\sem{\abststate} \subseteq \sem{\abststate'}$.
That is, it adjusts the abstraction precision of the given 
state~$\abststate$, resulting in a widened state~$\abststate'$ 
and a new abstraction precision~$\precision'$.
An abstraction is, for example, computed based on the abstraction
operator~$\abst{\cdot}^\precision$ with widening based on the
given abstraction precision~$\precision$.
Please note that the precision adjustment operator does not 
add any requirements 
on the given abstraction precision~$\precision$ and the returned 
abstraction precision~$\precision'$---while such a requirement 
can help to ensure the progress of the analysis.
\end{operator}

\begin{operator}{$\targetop$}
The \emph{target operator}~$\targetop: \abststates \rightarrow 2^\properties$ determines
if a given abstract state is a target state of the analysis process, for example,
a state that must not be reachable in the concrete system (safety property).
A call~$\targetop(\abststate)$ returns a set of properties~$\propertyset \subseteq \properties$ for that 
the given abstract state might have to be ruled out.
The operator returns the empty set~$\emptyset$ if the state is not a target state.
\end{operator}

\subsection{Composite CPA}
\label{sec:compositecpa}
\label{concept:composite}
In the framework of configurable program analysis~\cite{CPA} 
different analyses~(CPAs) can be responsible for tracking different 
facts about the system under analysis. 
We need a mechanism for composing different analyses, their 
abstract domains and semilattices, and operators.
This mechanism is provided by the \emph{Composite CPA}~\cite{CPA}.
A composite CPA~$\cpa_\times$ is composed of a sequence of 
\emph{component analyses}~$\vstart \cpa_1, \ldots, \cpa_n \vend$. 
The \emph{composite domain}~$\abstdomain_\times$ is the direct product
of the abstract domains of the component analysis 
domains~$\vstart \abstdomain_1, \ldots, \abstdomain_n \vend$, that is,
it operates on \emph{abstract composite 
states}~$\abststates_\times = \abststates_1 \times \ldots \times \abststates_n$,
which are elements of the \emph{product lattice}~$\lattice_\times = \lattice_1 \times \ldots \times \lattice_n$. 

\subsubsection{Strengthening}
Whenever an analysis runs as a component analysis within a composite analysis,
it can implement an additional strengthening operator~$\strengthen$.
The operator is invoked for each component analysis~$c_1, \ldots, c_n$ separately,
after all of them have computed a successor state based on their transfer relation,
which resulted in the composite state~$e_\times' = (e_1, \ldots, e_n)$. 
%
Compared to the original formalism~\cite{CPA,CPAplus}, we have extended
the strengthening operator for our needs. 
The remaining details about this analysis can be found 
in the literature~\cite{CPA,CPAplus}.

\begin{operator}{$\strengthen$}
The \emph{strengthening operator}~$\strengthen: E_\times \times E_\times \times E_{c_i} \rightarrow E_{c_i}$ 
can be implemented in a component analysis to use information from other 
abstract states in the composite state to strengthen the component state.
A call~$\strengthen_i(e_\times, e_\times', e_{c_i})$
takes as argument the predecessor composite state~$e_\times \in \abststates_\times$,
the successor composite state~$e_\times' \in \abststates_\times$, 
and the abstract component successor state~$e_{c_i} \in E_i$, and returns 
a strengthened successor state~$e_{c_i'} \in E_i$.
The strengthening process can take information from~$e_\times$ 
and~$e_\times'$ into account.
\end{operator}

\subsection{Predicate CPA}

We use the predicate abstraction with adjustable block encoding~\cite{ABE} 
to abstract the heap and stack of the program under analysis.
The functionality of this analysis is implemented in 
the~\emph{Predicate CPA}~$\cpa_\predcpa$.
We now describe those details of the analysis that are relevant 
for this work. 
Please refer to the literature~\cite{ABE} for a 
full description of this analysis.

\begin{component}{Abstract Domain $\abstdomain_\predcpa$}
The abstract domain~$\abstdomain_\predcpa = (\concstates, \mathcal{E}, \sem{\cdot})$
is defined based on a semilattice~$\mathcal{E}$ on the set of 
abstract states~$E = \formulas \times \formulas \times \locations$.
An abstract predicate state~$e = (\blockformula, \abstformula, \abstlocation) \in E$
consists of a \emph{block formula}~$\blockformula$, an 
\emph{abstraction formula}~$\abstformula$ (summary), and an 
\emph{abstraction location}~$\abstlocation \in \locations$.
The abstraction formula is typically stored in a BDD~\cite{AllSmt}, 
which allows fast entailment checks on the level of propositional 
variables, and simplifies the formulas. 

Details on the semilattice~$\mathcal{E}$ can be found in the literature~\cite{ABE}.
Since we use the Predicate CPA (and this abstract domain) in a 
composite analysis along with an analysis that keeps care of 
tracking the current position in the transition relation of the 
system under analysis, we do not model the current control 
location as part of this domain---as done in existing work~\cite{ABE}.
\end{component}

\begin{operator}{$\precop_\predcpa$}
We use the precision adjustment operator~$\precop_\predcpa: \abststates \times \precisions \times 2^{\abststates \times \precisions} \rightarrow \abststates \times \precisions$
to compute predicate abstractions, at specific control locations---%
called the abstraction locations.

The \emph{block operator}~$\blk: \abststates \times \locations \times \Bools$
\recap{Block Operator}
is used to determine the points in the state space for that an 
abstraction~(summary) should be computed based on a given 
abstraction precision (set of predicates). 
The block operator~$\blk_\textit{L}$ returns \true iff the given 
control location is a loop head, the block operator~$\blk_\textit{LF}$ 
returns \true iff the given control location is a function call 
or a loop head, and the operator
$\blk_\textit{SBE}$ returns \true always, that is, 
fosters a single-block encoding~\cite{LBE,BooleanCartesian}.
Cartesian predicate abstraction is used to compute the abstraction in case
single-block encoding~\cite{BooleanCartesian} is enabled;
otherwise, Boolean predicate abstraction~\cite{AllSmt} is used.
Please note that the original analysis~\cite{ABE} computes abstraction in the 
transfer relation of the analysis.

Given an abstract state~$e = (\blockformula, \abstformula, \abstlocation)$
and a set of predicate~$\precision$ for a control 
location~$\location \in \locations$, the operator~$\precop_\predcpa$
returns $(e, \precision)$ if $\blk(e,\location) = \false$, otherwise,
it returns~$((\true, \abst{\abstformula \land \blockformula}^\precision, \location), \precision)$.
Depending on the block operator, a different abstraction 
function~$\abst{\cdot}^\precision$ with widening is used to 
conduct either a Cartesian predicate abstraction or a 
Boolean predicate abstraction.
\end{operator}


==> text/explicitstutter.tex <==
\begin{figure}[tp]
\begin{subfigure}[b]{.20\linewidth}
\centering
\begin{tikzpicture}[node distance=8mm, scale=0.7, transform shape]
\node[cfastate] (q0) {$q_0$};
\node[cfastate,below left=of q0] (q1) {$q_1$};
\node[cfastate,below=of q1] (q2) {$q_2$};
\node[cfatargetstate,below=of q2] (q3) {$q_3$};
\node[cfastate,below right=of q0] (q4) {$q_4$};
\node[cfastate,below=of q4] (q5) {$q_5$};
\node[cfatargetstate,below=of q5] (q6) {$q_6$};

\path[trans,one] (q0) edge node [pos=.5,label=left:{$\epsilon$}] {} (q1);
\path[trans,one] (q1) edge node [pos=.5,label=left:{$\srccode{a}$}] {} (q2);
\path[trans,one] (q2) edge node [pos=.5,label=left:{$\srccode{b}$}] {} (q3);

\path[trans,two] (q0) edge node [pos=.5,label=right:{$\epsilon$}] {} (q4);
\path[trans,two] (q4) edge node [pos=.5,label=right:{\srccode{f}}] {} (q5);
\path[trans,two] (q5) edge node [pos=.5,label=right:{\srccode{g}}] {} (q6);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\begin{subfigure}[b]{.20\linewidth}
\centering
\begin{tikzpicture}[node distance=8mm, scale=0.7, transform shape]
\node[cfastate] (q0) {$q_0$};
\node[below left=of q0] (q1) {};
\node[cfastate,below=of q1] (q2) {$q_2$};
\node[cfatargetstate,below=of q2] (q3) {$q_3$};
\node[below right=of q0] (q4) {};
\node[cfastate,below=of q4] (q5) {$q_5$};
\node[cfatargetstate,below=of q5] (q6) {$q_6$};

\path[trans,one] (q0) edge node [pos=.5,label=left:{$\srccode{a}$}] {} (q2);
\path[trans,one] (q2) edge node [pos=.5,label=left:{$\srccode{b}$}] {} (q3);

\path[trans,two] (q0) edge node [pos=.5,label=right:{$\srccode{f}$}] {} (q5);
\path[trans,two] (q5) edge node [pos=.5,label=right:{$\srccode{g}$}] {} (q6);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\begin{subfigure}[b]{.28\linewidth}
\centering
\begin{tikzpicture}[node distance=8mm, scale=0.7, transform shape]
\node[cfastate] (q0) {$q_0$};
\node[cfastate,below left=of q0] (q1) {$q_1$};
\node[cfastate,below=of q1] (q2) {$q_2$};
\node[cfatargetstate,below=of q2] (q3) {$q_3$};
\node[cfastate,below right=of q0] (q4) {$q_4$};
\node[cfastate,below=of q4] (q5) {$q_5$};
\node[cfatargetstate,below=of q5] (q6) {$q_6$};

\path[trans,one] (q0) edge node [pos=.5,label=left:{$\epsilon$}] {} (q1);
\path[trans,one] (q1) edge node [pos=.5,label=left:{$\srccode{a}$}] {} (q2);
\path[trans,one] (q2) edge node [pos=.5,label=left:{$\srccode{b}$}] {} (q3);

\path[trans,one] (q1) edge [loop left] node [anchor=center,left] {\textsf{else}} (q1);
\path[trans,one] (q2) edge [loop left] node [anchor=center,left] {\textsf{else}} (q2);

\path[trans,two] (q0) edge node [pos=.5,label=right:{$\epsilon$}] {} (q4);
\path[trans,two] (q4) edge node [pos=.5,label=right:{\srccode{f}}] {} (q5);
\path[trans,two] (q5) edge node [pos=.5,label=right:{\srccode{g}}] {} (q6);

\path[trans,two] (q4) edge [loop right] node [anchor=center,right] {\textsf{else}} (q4);
\path[trans,two] (q5) edge [loop right] node [anchor=center,right] {\textsf{else}} (q5);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\begin{subfigure}[b]{.28\linewidth}
\centering
\begin{tikzpicture}[node distance=8mm, scale=0.7, transform shape]
\node[cfastate] (q0) {$q_0$};
\node[cfastate,below left=of q0] (q1) {$q_1$};
\node[cfastate,below=of q1] (q2) {$q_2$};
\node[cfatargetstate,below=of q2] (q3) {$q_3$};
\node[cfastate,below right=of q0] (q4) {$q_4$};
\node[cfastate,below=of q4] (q5) {$q_5$};
\node[cfatargetstate,below=of q5] (q6) {$q_6$};

\path[trans,one] (q0) edge node [pos=.5,label=left:{$\lnot \srccode{a}$}] {} (q1);
\path[trans,one] (q1) edge node [pos=.5,label=left:{$\srccode{a}$}] {} (q2);
\path[trans,one] (q2) edge node [pos=.5,label=left:{$\srccode{b}$}] {} (q3);

\path[trans,one] (q0) edge node [pos=.7,label=right:{\srccode{a}}] {} (q2);

\path[trans,one] (q1) edge [loop left] node [anchor=center,left] {\textsf{else}} (q1);
\path[trans,one] (q2) edge [loop left] node [anchor=center,left] {\textsf{else}} (q2);

\path[trans,two] (q0) edge node [pos=.5,label=right:{$\lnot \srccode{f}$}] {} (q4);
\path[trans,two] (q4) edge node [pos=.5,label=right:{\srccode{f}}] {} (q5);
\path[trans,two] (q5) edge node [pos=.5,label=right:{\srccode{g}}] {} (q6);

\path[trans,two] (q0) edge node [pos=.7,label=left:{\srccode{f}}] {} (q5);

\path[trans,two] (q4) edge [loop right] node [anchor=center,right] {\textsf{else}} (q4);
\path[trans,two] (q5) edge [loop right] node [anchor=center,right] {\textsf{else}} (q5);
\end{tikzpicture}
\caption{}
\end{subfigure}
\caption{An explicit modeling of stuttering transitions is needed for elimination 
of $\epsilon$--transitions. 
Automaton~(b) is the result of eliminating the $\epsilon$--transitions from 
automaton~(a), automaton~(d) is the result for automaton~(c), respectively.
We assume all automata to have a language that is invariant under stuttering.
Automaton~(b) cannot recognize the word~$\vstart \srccode{a}, \srccode{f}, \srccode{g} \vend$ 
since it would first enter state~$q_2$ and then only accept the symbol~$\srccode{b}$ 
to get to the accepting target state~$q_3$.
It is sufficient to add explicitly stuttering transitions to closure termination
states only, that is, to control states~$q_1$ and $q_4$, before conducting the $\epsilon$--elimination.
}
\label{fig:stutteringtreatment}
\end{figure}


==> text/productexample.tex <==
\begin{figure}[tp]
%
\begin{subfigure}[b]{.49\linewidth}
\centering
\begin{tikzpicture}[node distance=12mm, scale=0.7, transform shape,auto]
\node[] at (0.5,0.5) (top) {};
\node[] at (0.5,-8) (bottom) {};

\node[] (qs) {};
\node[] at (0,-8) (ql) {$~$};
\node[cfastate,below of=qs,minimum size=8mm] (q1) {$q_1$};
\node[cfastate,below=of q1,minimum size=8mm] (q2) {$q_2$};
\node[cfatargetstate,below=of q2,minimum size=8mm] (q3) {$q_3$};
\node[cfatargetstate,below=of q3,minimum size=8mm] (q4) {$q_4$};

\path[trans,two] (q1) edge [loop left] node [anchor=center,left] {\textsf{else}} (q1);
\path[trans,two] (q2) edge [loop right] node [anchor=center,right] {\textsf{else}} (q2);

\path[trans] (qs) edge [] node [anchor=center,above] {} (q1);

\path[trans,two] (q1) edge [bend right] node [anchor=center,right] {$a$} (q2);
\path[trans,two] (q2) edge [] node [anchor=center,left] {$a$} (q3);
\path[trans,two] (q2) edge [bend right] node [anchor=center,right] {$b$} (q1);
\path[trans,two] (q1) edge [bend right] node [anchor=center,left] {$b$} (q4);
\end{tikzpicture}
%
\begin{tikzpicture}[node distance=12mm, scale=0.7, transform shape,auto]
\node[] at (0.7,0.5) (top) {};
\node[] at (0.7,-8) (bottom) {};

\node[] (qs) {};
\node[] at (0,-8) (ql) {$~$};
\node[cfastate,below of=qs,minimum size=8mm] (q1) {$q_5$};
\node[cfastate,below=of q1,minimum size=8mm] (q2) {$q_6$};
\node[cfatargetstate,below=of q2,minimum size=8mm] (q3) {$q_7$};
\node[cfatargetstate,below=of q3,minimum size=8mm] (q4) {$q_8$};

\path[trans,one] (q1) edge [loop left] node [anchor=center,left] {\textsf{else}} (q1);
\path[trans,one] (q2) edge [loop right] node [anchor=center,right] {\textsf{else}} (q2);

\path[trans] (qs) edge [] node [anchor=center,above] {} (q1);

\path[trans,one] (q1) edge [bend right] node [anchor=center,right] {$c$} (q2);
\path[trans,one] (q2) edge [] node [anchor=center,left] {$c$} (q3);
\path[trans,one] (q2) edge [bend right] node [anchor=center,right] {$d$} (q1);
\path[trans,one] (q1) edge [bend right] node [anchor=center,left] {$d$} (q4);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\begin{subfigure}[b]{.49\linewidth}
\centering
\begin{tikzpicture}[node distance=12mm, scale=0.7, transform shape,auto]

\node[] at (1.8,0.5) (top) {};
\node[] at (1.8,-9) (bottom) {};

\node[] (qs) {};
\node[] at (0,-9) (ql) {$~$};
\node[cfastate,below of=qs,minimum size=8mm] (q0) {$q_0$};

\path[trans] (qs) edge [] node [anchor=center,above] {} (q0);

\node[cfastate,minimum size=8mm] at (-1.4,-2) (q1) {$q_1$};
\node[cfastate,below=of q1,minimum size=8mm] (q2) {$q_2$};
\node[cfatargetstate,below=of q2,minimum size=8mm] (q3) {$q_3$};
\node[cfatargetstate,below=of q3,minimum size=8mm] (q4) {$q_4$};

\node[cfastate,minimum size=8mm] at (1.4,-2) (q5) {$q_5$};
\node[cfastate,below=of q5,minimum size=8mm] (q6) {$q_6$};
\node[cfatargetstate,below=of q6,minimum size=8mm] (q7) {$q_7$};
\node[cfatargetstate,below=of q7,minimum size=8mm] (q8) {$q_8$};

\path[trans,two] (q1) edge [loop left] node [anchor=center,left] {\textsf{else}} (q1);
\path[trans,two] (q2) edge [loop right] node [anchor=center,right] {\textsf{else}} (q2);

\path[trans,one] (q5) edge [loop left] node [anchor=center,left] {\textsf{else}} (q5);
\path[trans,one] (q6) edge [loop right] node [anchor=center,right] {\textsf{else}} (q6);


\path[trans,two] (q1) edge [bend right] node [anchor=center,right] {$a$} (q2);
\path[trans,two] (q2) edge [] node [anchor=center,left] {$a$} (q3);
\path[trans,two] (q2) edge [bend right] node [anchor=center,right] {$b$} (q1);
\path[trans,two] (q1) edge [bend right] node [anchor=center,left] {$b$} (q4);

\path[trans,one] (q5) edge [bend right] node [anchor=center,right] {$c$} (q6);
\path[trans,one] (q6) edge [] node [anchor=center,left] {$c$} (q7);
\path[trans,one] (q6) edge [bend right] node [anchor=center,right] {$d$} (q5);
\path[trans,one] (q5) edge [bend right] node [anchor=center,left] {$d$} (q8);

\path[trans] (q0) edge [bend right] node [anchor=center,above] {$\epsilon$} (q1);
\path[trans] (q0) edge [bend left] node [anchor=center,above] {$\epsilon$} (q5);
\end{tikzpicture}
\caption{}
\end{subfigure}

\begin{subfigure}[b]{.49\linewidth}
\centering
\begin{tikzpicture}[node distance=12mm, scale=0.7, transform shape,auto]

\node[] at (1.8,0.5) (top) {};
\node[] at (1.8,-9) (bottom) {};

\node[] (qs) {};
\node[] at (0,-9) (ql) {$~$};
\node[cfastate,below of=qs,minimum size=8mm] (q0) {$q_0$};

\path[trans] (qs) edge [] node [anchor=center,above] {} (q0);

\node[cfatargetstate,minimum size=8mm] at (-2,-2) (q4) {$q_4$};
\node[cfastate,below=of q4,minimum size=8mm] (q1) {$q_1$};
\node[cfastate,minimum size=8mm] at (-1.5,-6) (q2) {$q_2$};
\node[cfatargetstate,below=of q2,minimum size=8mm] (q3) {$q_3$};

\node[cfatargetstate,minimum size=8mm] at (2,-2) (q8) {$q_8$};
\node[cfastate,below=of q8,minimum size=8mm] (q5) {$q_5$};
\node[cfastate,minimum size=8mm] at (1.5,-6) (q6) {$q_6$};
\node[cfatargetstate,below=of q6,minimum size=8mm] (q7) {$q_7$};

\path[trans,two] (q1) edge [loop left] node [anchor=center,left] {$\lnot (a \lor b)$} (q1);
\path[trans,two] (q2) edge [loop left] node [anchor=center,left] {$\lnot (a \lor b)$} (q2);

\path[trans,one] (q5) edge [loop right] node [anchor=center,right] {$\lnot (c \lor d)$} (q5);
\path[trans,one] (q6) edge [loop right] node [anchor=center,right] {$\lnot (c \lor d)$} (q6);

\path[trans,two] (q0) edge [sloped] node [anchor=center,above] {$\lnot (a \lor b)$} (q1);
\path[trans,one] (q0) edge [sloped] node [anchor=center,above] {$\lnot (c \lor d)$} (q5);


\path[trans,two] (q1) edge [bend right] node [anchor=center,left] {$a$} (q2);
\path[trans,two] (q2) edge [] node [anchor=center,left] {$a$} (q3);
\path[trans,two] (q2) edge [bend right] node [anchor=center,left] {$b$} (q1);
\path[trans,two] (q1) edge [] node [anchor=center,left] {$b$} (q4);

\path[trans,one] (q5) edge [bend right] node [anchor=center,right] {$c$} (q6);
\path[trans,one] (q6) edge [] node [anchor=center,right] {$c$} (q7);
\path[trans,one] (q6) edge [bend right] node [anchor=center,right] {$d$} (q5);
\path[trans,one] (q5) edge [] node [anchor=center,right] {$d$} (q8);

\path[trans,two] (q0) edge [] node [anchor=center,above] {$b$} (q4);
\path[trans,one] (q0) edge [] node [anchor=center,above] {$d$} (q8);

\path[trans,two] (q0) edge [] node [anchor=center,left] {$a$} (q2);
\path[trans,one] (q0) edge [] node [anchor=center,right] {$c$} (q6);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\begin{subfigure}[b]{.49\linewidth}
\centering
\begin{tikzpicture}[node distance=12mm, scale=0.7, transform shape,auto]
\node[] (qs) {};

\node[cfastate,below=of qs] (q15) {$q_{1|5}$};
\node[cfastate,right=of q15] (q16) {$q_{1|6}$};
\node[cfatargetstate,right=of q16] (q17) {$q_{1|7}$};
\node[cfatargetstate,right=of q17] (q18) {$q_{1|8}$};

\node[cfastate,below=of q15]  (q25) {$q_{2|5}$};
\node[cfastate,right=of q25] (q26) {$q_{2|6}$};
\node[cfatargetstate,right=of q26] (q27) {$q_{2|7}$};
\node[cfatargetstate,right=of q27] (q28) {$q_{2|8}$};

\node[cfatargetstate,below=of q25]  (q35) {$q_{3|5}$};
\node[cfatargetstate,right=of q35] (q36) {$q_{3|6}$};
\node[cfatargetstate,right=of q36] (q37) {$q_{3|7}$};
\node[cfatargetstate,right=of q37] (q38) {$q_{3|8}$};

\node[cfatargetstate,below=of q35]  (q45) {$q_{4|5}$};
\node[cfatargetstate,right=of q45] (q46) {$q_{4|6}$};
\node[cfatargetstate,right=of q46] (q47) {$q_{4|7}$};
\node[cfatargetstate,right=of q47] (q48) {$q_{4|8}$};

\path[trans] (qs) edge [] node [anchor=center,above] {} (q15);

\path[trans,two] (q15) edge [bend right] node [anchor=center,left] {$a$} (q25);
\path[trans,two] (q16) edge [bend right] node [anchor=center,left] {$a$} (q26);
\path[trans,two] (q17) edge [bend right] node [anchor=center,left] {$a$} (q27);
\path[trans,two] (q18) edge [bend right] node [anchor=center,left] {$a$} (q28);

\path[trans,two] (q15) edge [bend right] node [anchor=center,left] {$b$} (q45);
\path[trans,two] (q16) edge [bend right] node [anchor=center,left] {$b$} (q46);
\path[trans,two] (q17) edge [bend right] node [anchor=center,left] {$b$} (q47);
\path[trans,two] (q18) edge [bend right] node [anchor=center,left] {$b$} (q48);

\path[trans,two] (q25) edge [bend right] node [anchor=center,left] {$b$} (q15);
\path[trans,two] (q26) edge [bend right] node [anchor=center,left] {$b$} (q16);
\path[trans,two] (q27) edge [bend right] node [anchor=center,left] {$b$} (q17);
\path[trans,two] (q28) edge [bend right] node [anchor=center,left] {$b$} (q18);

\path[trans,two] (q25) edge [] node [anchor=center,left] {$a$} (q35);
\path[trans,two] (q26) edge [] node [anchor=center,left] {$a$} (q36);
\path[trans,two] (q27) edge [] node [anchor=center,left] {$a$} (q37);
\path[trans,two] (q28) edge [] node [anchor=center,left] {$a$} (q38);

\path[trans,one] (q15) edge [bend right] node [anchor=center,above] {$c$} (q16);
\path[trans,one] (q25) edge [bend right] node [anchor=center,above] {$c$} (q26);
\path[trans,one] (q35) edge [bend right] node [anchor=center,above] {$c$} (q36);
\path[trans,one] (q45) edge [bend right] node [anchor=center,above] {$c$} (q46);

\path[trans,one] (q16) edge [] node [anchor=center,above] {$c$} (q17);
\path[trans,one] (q26) edge [] node [anchor=center,above] {$c$} (q27);
\path[trans,one] (q36) edge [] node [anchor=center,above] {$c$} (q37);
\path[trans,one] (q46) edge [] node [anchor=center,above] {$c$} (q47);

\path[trans,one] (q16) edge [bend right] node [anchor=center,above] {$d$} (q15);
\path[trans,one] (q26) edge [bend right] node [anchor=center,above] {$d$} (q25);
\path[trans,one] (q36) edge [bend right] node [anchor=center,above] {$d$} (q35);
\path[trans,one] (q46) edge [bend right] node [anchor=center,above] {$d$} (q45);

\path[trans,one] (q15) edge [bend right] node [anchor=center,above] {$d$} (q18);
\path[trans,one] (q25) edge [bend right] node [anchor=center,above] {$d$} (q28);
\path[trans,one] (q35) edge [bend right] node [anchor=center,above] {$d$} (q38);
\path[trans,one] (q45) edge [bend right] node [anchor=center,above] {$d$} (q48);
\end{tikzpicture}
\caption{}
\end{subfigure}
%
\caption{Example to illustrate an union of two automata~(a)---for 
transducers, also the output has to be considered.
One approach~\cite{Sipser} is to take advantage of $\epsilon$--transitions, 
which results in the non-deterministic automaton~(b).
The $\epsilon$--transitions can get removed, which results in 
the non-deterministic automaton~(c).
An alternative is to explicitly construct the deterministic 
product automaton~(d), based on a powerset (or subset) construction, 
which can have an exponential number of states.
Please note: That we have \emph{not drawn the stuttering self transitions}
that are present for each of the control states in automaton~(d).}
\label{fig:automata:union}
\end{figure}


==> text/reducealg.tex <==
\begin{algorithm}[t]
\begin{small}
    \caption{$\reduceop_\text{Left}(\transducer_\epsilon)$}
\label{alg:reduce}
\begin{algorithmic}[1]
\vspace{1mm}
\INPUT Abstract transducer~$\transducer_\epsilon \in \transducers$ \\
\vspace{1mm}
\OUTPUT Abstract transducer~$\transducer \in \transducers$, 
    with~$\langacc(\transducer_\epsilon) = \langacc(\transducer)$ 
    and $\transductions(\transducer_\epsilon) = \transductions(\transducer)$
\vspace{1mm}
\newline
\COMMENT{// Ensure that the transducer is input--$\epsilon$--free}
\STATE $(\atmtstates, \inputdomain, \outputdomain, 
    \atmtinit, \atmtfinal, \atmtrelation) = \textsf{elim}(\transducer_\epsilon)$ 
\newline
\COMMENT{// Initial equivalence relation (partitioning)}
\STATE $Q_\equiv = \{ \; (q, q) \; \; | \; q \in \atmtstates \; \} $
\newline
\COMMENT{// Initial worklist}
\STATE $W = \{ q \; | \; (q, \inputlang) \in \atmtinit \; \}$
\newline
\COMMENT{// Build the left-equivalence relation}
\WHILE {$W \neq \emptyset$}
    \STATE $w = W.\textsf{pop()}$
    \FOR {$\inputlang \in \{ \; \inputlang \; | \; (w, \inputlang, q', \outputlang) \in \atmtrelation \; \} $}
        \STATE $S = \{ \; q' \; 
            | \; (w, \inputlang_t, q') \land \sem{\inputlang}_\inputcomp = \sem{\inputlang_t}_\inputcomp \; \} $
        \STATE $Q_\equiv = Q_\equiv \cup \{ (q_1, q_2) \; | \; q_1, q_2 \in S \; \}$
        \STATE $W = W \cup S\ $
    \ENDFOR
\ENDWHILE
\STATE \textbf{return} $(\atmtstates, \inputdomain, 
    \outputdomain, \atmtinit', \atmtfinal, \atmtrelation')$
\end{algorithmic}
\vspace{1mm}
\end{small}
\end{algorithm}


==> text/transferalg.tex <==
\begin{algorithm}[t]
\begin{small}
\caption{$\transabs{}{}_\transcpa(\transducerss, \inputlang, \precision)$}
\label{alg:transducer:transfer}
\begin{algorithmic}[1]
\vspace{1mm}
\INPUT A transducer state set~$\transducerss \subseteq \absttransducerstates$, \\
\hspace{5mm}      an input language~$\inputlang \in \inputlangs$,  \\
\hspace{5mm}      an abstraction precision~$\precision \in \precisions_\transducer$,  \\
\hspace{5mm}      and a transducer~$\transducer \in \transducers$ as implicit parameter.  \\
\vspace{1mm}
\OUTPUT A set of abstract transducer states~$\subseteq \absttransducerstates$
\vspace{1mm}
\STATE $\Delta = \emptyset$
\FOR {$(q, \outputlang) \in \outclosure_\precision(\transducerss)$}
  \FOR {$\transtrans = (q, \inputlang', q', \outputlang') \in \atmtrelation$}
    \IF {$\inputlang' \less \inputlang$}
        \STATE $\Delta = \Delta \cup \{ (q, \outputlang, q', \outputlang \concat \outputlang') \}$
    \ENDIF
  \ENDFOR
\ENDFOR
\STATE \textbf{ return } $\{ \; \stateadjust(\tau) \; | \; \tau \in \Delta \; \}$
\end{algorithmic}
\vspace{1mm}
\end{small}
\end{algorithm}


==> text/worddomain.tex <==
\subsection{Abstract Word Domain}

\begin{definition}[Abstract Word Lattice.]The \emph{abstract word lattice} of an abstract word domain~\abstworddomain 
is lattice~$$\abstractwordlattice = (\abstractwords, \abstless, \abstmeet, \abstjoin, \absttop, \abstbot)$$
that describes the relationship between the abstract words in the set~\abstractwords. 
One abstract word~$\abstractword \in \abstractwords$ describes 
a set of concrete words, that is, $\sem{\abstractword} \subseteq \concretewords$.
The inclusion relation~$\abstless \subseteq \abstractwords \times \abstractwords$ has the 
element~$(\abstractword_1, \abstractword_2) \in \abstless$ if and only if 
for each~$\concreteword_1 \in \sem{\abstractword_1}$ there is
an element~$\concreteword_2 \in \sem{\abstractword_2}$ 
with~$\concreteword_1 \less \concreteword_2$.
The definition of the least upper bound (join)~\abstjoin, and the 
greatest lower bound (meet)~\abstmeet follow from the definition
of the inclusion relation~\abstless.
The top element~$\absttop$ represents the set of all words, 
that is, $\sem{\absttop} = \concretes^*$ and for 
each~$\abstractword \in \abstractwords$ holds true 
that~$(\abstractword, \absttop) \in \abstless$.
The bottom element~$\abstbot$ represents the empty word, 
that is, $\sem{\abstbot} = \{ \epsilon \}$, that is,
the abstract word~\abstbot is prefix of any other abstract 
word~$\abstractword \in \abstractwords$,
that is, $(\abstbot, \abstractword) \in \less$.
\end{definition}

\subsection{Product of Abstract Word Domains}
\label{sec:artifact:compositedomain}%

Abstract word artifacts of different types~$\artefacts_1, \artefacts_2 \subseteq \artefacts$ 
and their respective abstract word domains~$\abstworddomain_{\artefacts_1}$ 
and $\abstworddomain_{\artefacts_2}$ can be combined to form compound word domains.
A compound word domain is a product domain~\cite{SemanticDomains}~$\abstworddomain_\times = \abstworddomain_{\artefacts_1} \times \abstworddomain_{\artefacts_2}$ 
on compound word artifacts~$\artefacts_\times \subseteq \artefacts_1 \times \artefacts_2$.
Please note that also compound word artifacts are abstract word artifacts.
An abstract word artifact~$\artifact_1$ \emph{overapproximates} a word
artifact~$\artifact_2$ if and only if~$\sem{\artifact_2} \subseteq \sem{\artifact_1}$.

We assume that any existing abstract domain can get 
\emph{lifted}~\cite{GallJeannet2007} to become an abstract word domain.


At certain points in an analysis process, a means for combining entities
of different type is needed to share them as one (compound) entity.
We distinguish between two types of combined abstract words: 
orthogonal and composite words. 
This types of abstract words are distinguished by their denotation~(their 
semantics), that is, both are pairs of abstract words but one represents
the union and the other the intersection of the corresponding sets
of concrete words:

\begin{definition}[Composite Word Domain]A \emph{composite word domain} composes to abstract word domains as composites,
that is, the \emph{intersection of the semantics} of the composed abstract words is 
constructed---a strengthening is conducted;
it maps between composite word artifacts and concrete word artifacts.
\end{definition}

\begin{definition}[Composite Word.]A \emph{composite word}~$\artifact_c = (\artifact_1, \artifact_2) \in \artifacts_1 \times \artifacts_2 \in \artifacts$
is an abstract word that (1)~pairs two abstract of possibly
different types, (2)~while \emph{intersecting their semantics}, that is, 
$\sem{\artifact_c} = \sem{(\artifact_1, \artifact_2)} = \sem{\artifact_1} \cap \sem{\artifact_2}$.
\end{definition}

\begin{definition}[Concurrent Word Domain]A \emph{orthogonal word domain} composes to abstract word domains such that 
the \emph{union of the semantics} of the composed abstract words is 
constructed---a different symbolic representation that neither adds nor removes 
information is conducted; 
it maps between orthogonal word artifacts and concrete word artifacts.
\end{definition}

\begin{definition}[Concurrent Word.]An \emph{orthogonal word}~$\artifact_o = (\artifact_1, \artifact_2) \in \artifacts_1 \times \artifacts_2 \in \artifacts$
is an abstract word that (1)~pairs two abstract words of possibly
different types, while (2)~keeping them \emph{semantically independent}, that is, 
$\sem{\artifact_o} = \sem{(\artifact_1, \artifact_2)} = \sem{\artifact_1} \times \sem{\artifact_2}$.
\end{definition}

We use the constructor~$\cup: \artifacts \times \artifacts \rightarrow \artifacts$ to
create an orthogonal words from two given abstract words.
The constructor~$\cap: \artifacts \times \artifacts \rightarrow \artifacts$ is used
to create the respective composite words.

